Connectivity graphs of uncertainty regions

We study connectivity relations among points, where the precise location of each input point lies in a region of uncertainty. We distinguish two fundamental scenarios under which uncertainty arises. In the favorable Best-Case Uncertainty (BU), each input point can be chosen from a given set to yield the best possible objective value. In the unfavorable Worst-Case Uncertainty (WU), the input set has worst possible objective value among all possible point locations, which are uncertain due, for example, to imprecise data. We consider these notions of uncertainty for the bottleneck spanning tree problem, giving rise to the following Best-Case Connectivity with Uncertainty (BCU) problem: Given a family of geometric regions, choose one point per region, such that the longest edge length of an associated geometric spanning tree is minimized. We show that this problem is NP-hard even for very simple scenarios in which the regions are line segments or squares. On the other hand, we give an exact solution for the case in which there are n+k regions, where k of the regions are line segments and n of the regions are fixed points. We then give approximation algorithms for cases where the regions are either all line segments or all unit discs. We also provide approximation methods for the corresponding Worst-Case Connectivity with Uncertainty (WCU) problem: Given a set of uncertainty regions, find the minimal distance r such that for any choice of points, one per region, there is a spanning tree among the points with edge length at most r.

==> abstract.tex <==
We study connectivity relations among points, where the precise
location of each input point lies in a region of uncertainty. We
distinguish two fundamental scenarios under which uncertainty arises.
In the favorable {\em Best-Case Uncertainty} (BU), each input point
can be chosen from a given set to yield the best possible objective
value.  In the unfavorable {\em Worst-Case Uncertainty} (WU), the
input set has worst possible objective value among all possible point
locations, which are uncertain due, for example, to imprecise data.

%We consider these notions of uncertainty for the bottleneck spanning tree problem,
%given rise to 
%{\em Best-Case Connectivity with Uncertainty} (BCU) as follows. 
%Given a family of geometric regions, choose one point per region, such that the longest length of 
%an associated geometric spanning tree is minimized.
We consider these notions of uncertainty for the bottleneck spanning
tree problem, giving rise to the following {\em Best-Case Connectivity
  with Uncertainty} (BCU) problem: Given a family of geometric
regions, choose one point per region, such that the longest edge
length of an associated geometric spanning tree is minimized.  We show
that this problem is NP-hard even for very simple scenarios in which
the regions are line segments or squares.  On the other hand, we give
an exact solution for the case in which there are $n+k$ regions, where
$k$ of the regions are line segments and $n$ of the regions are fixed
points.  We then give approximation algorithms for cases where the
regions are either all line segments or all unit discs. We also
provide approximation methods for the corresponding {\em Worst-Case
  Connectivity with Uncertainty} (WCU) problem: Given a set of
uncertainty regions, find the minimal distance $r$ such that for any
choice of points, one per region, there is a spanning tree among the
points with edge length at most $r$.



==> algorithm.tex <==
% !TEX root = uncertainalpha_journal.tex
\section{An Exact Algorithm for Solving BCU for $n$ Fixed Points and $k$ Segments}\label{sec:exactAlgorithm}

We present an exact algorithm that solves BCU---for a given precision
$\delta$---when the input consist of $n$ fixed points, and the
uncertainty regions are $k$ line segments, possibly of varying length,
in general position. That is, no two of the line segments are
parallel.  Our algorithm determines, in a time that is polynomial in
$n$ for any fixed $k$ and constant precision $\delta$, a set of point
positions on the line segments that permits a spanning tree whose
longest edge is of minimum length amongst all spanning trees that
connect exactly one point from each segment as well as all fixed
points.

Rather than give a practical algorithm, the aim of this section is to
show that BCU is indeed computable and provide an upper bound on the
running time.  Nevertheless, we introduce two tools below, minimum
solution trees and critical paths, in order to discretize and prune
the search space (over all possible labelled spanning trees on $n+k$
vertices) considerably.

We highlight in the Key ideas how the general position assumption
simplifies the proof of correctness of the algorithm, but the
extension to inputs that include parallel line segments is not
difficult to conceive.  We omit the details of such an extension for
the sake of clarity.


\subsubsection*{Key Ideas}
In our search for an optimum solution we focus on determining optimum
solutions that satisfy slightly stronger additional properties: we
seek a selection of point locations on the line segments which
supports a {\em minimum solution tree}.  A minimum solution tree is a
spanning tree for segment locations and fixed points that does not
just have a shortest longest edge, but also has a shortest second
longest edge amongst all such solutions, and so forth. Looking for
minimum solution trees, instead of optimum solutions, can decrease the
search space considerably by virtue of the fact that for certain
problem instances an infinite number of optimum solutions exist due to
freedom of point selection on the line segments.
%since due to freedom of point selection on the line segments, for certain instances an infinite number of optimum solutions exists.

{\em Critical paths} give support when determining minimum solution
trees. These are paths in spanning trees where all edges are of equal
length and all inner path points are located on line segments.
Further, moving the location of any of the points on segments will
lengthen at least one of the edges while shortening another.  

Our algorithm determines point locations on all segments that support
a minimum solution tree with longest tree edge of length $2\alpha$ as
follows. We enumerate candidates for critical paths, from longest to
shortest in terms of path length. Each candidate path is tested to see
whether or not it supports a critical path. If successful, and if the
edge length of this critical path is no longer than the longest edge
of the solution tree for the best point set found so far, the line
segments of that critical path are replaced by their corresponding
point locations.  The general position assumption provides that these
point locations are unique, and simplifies our method of computing
them.  We then recurse on the updated input.  Once all points on
segments are determined, a greedy algorithm to determine the
corresponding minimum solution tree can be applied.

\subsubsection*{Minimum Solution Trees}
To describe minimum solution trees formally, we begin by defining a
way that allows us to compare different spanning trees that correspond
to optimum solutions. We partition into equivalence classes the set of
all spanning trees taken over all fixed points and all point choices
on the $k$ segments, and we define a linear ordering on the
equivalence classes such that a minimum solution tree is a smallest
spanning tree w.r.t.~the linear ordering.

For any two selections of points on the $k$ segments, and for any two of their corresponding spanning trees, let ${\cal L}$ and ${\cal L'}$ be ordered lists of lengths of all edges in the two trees, sorted from longest to shortest. That is, ${\cal L}=(l_1,l_2,\ldots,l_{n+k-1})$ and ${\cal L'}=(l'_1,l'_2,\ldots,l'_{n+k-1})$, with $l_i\geq l_{i+1}$ and $l'_i\geq l'_{i+1}$ for all $i$.
%
We say that ${\cal L}$ \emph{is preferred over} ${\cal L'}$ if for a
certain $i$, $l_i<l'_i$, and $l_j=l'_j$ for all $j<i$.  If $\cal T$
and $\cal T'$ are spanning trees with edge lists $\cal L$ and
$\cal L'$, respectively, we also say $\cal T$ is preferred over
$\cal T'$ if $\cal L$ is preferred over $\cal L'$.
%
%ALEJANDRO:  I think this is more clear.
Note that this defines a linear ordering on lists in general, and not
only those derived from spanning tree edge-lengths.

Our algorithm seeks to choose points on segments that result in a
spanning tree such that no other spanning tree is preferred over it.
% preferred over \emph{all other possibilities} of point selections on the segments.
%
 We call such a tree a \emph{minimum solution tree} ${\cal T}$.\footnote{We remark that for lists ${\cal L}$ and ${\cal L'}$ for two different spanning trees with two different sets of points on the segments, it is possible that ${\cal L} = {\cal L'}$, so that optimum solutions that permit minimum solutions trees are in general not unique.} We call a choice of points on segments that results in a minimum solution tree  ${\cal T}$  a \emph{best point set} for  ${\cal T}$.

In a minimum solution tree ${\cal T}$, not only are longest edges as short as possible, but also the number of longest edges is minimum. In other words, a tree with a smallest number of shortest longest edges is preferred over the ones with more edges of the same length.
%
Further, for all $i$ the $i^{th}$  longest edge is as small as possible, and the number of edges of that length is minimum.
%


The above conditions imply convenient properties on the best point set w.r.t.~a minimum solution tree.
%
Note that, for any point $p$ on a segment in a best point set, it is impossible to {\em improve} the solution by slightly moving $p$ on its segment; in fact, any perturbation of a point must lengthen at least one of the edges
that is longest among all edges incident to $p$.
%
We now list the possibilities for a point $p$ on a segment in a best point set (see Figure~\ref{fig:type}) in distinguishing three different types. Given a point $p$ on a segment, we call an edge $e$ that belongs to a minimum solution tree ${\cal T}$ incident to $p$ {\em  locally longest} if no other tree edge of ${\cal T}$ incident to $p$ is longer than $e$. Then, in a minimum solution tree the possibilities for a point located on a segment  w.r.t.~its locally longest edges are as follows.

\begin{figure}[h]%
%
\centerline{%
\input{figureAlgorithmAa.tex}%
\input{figureAlgorithmAb.tex}%
\input{figureAlgorithmAc.tex}%
}%
\caption{Points (in \bluecolour) of Type $1$, $2$, and $3$ respectively, with the segment shown in bold,  incident edges in \bluecolour, and perpendicular (to the segment) shown in gray. In each case, moving the point along the segment results in a longer locally longest incident edge.}%
\label{fig:type}%
\end{figure}%

\begin{description}
\item[Type~1] Point $p$ lies at an extremity of the segment. Then,
  one of the locally longest edge, $e$, incident to $p$  lies on
  the half plane that is delimited by a line perpendicular to the segment and
  does not contain the segment.
  %
  We observe that moving $p$ would lengthen $e$.
 %
\item[Type~2] Point $p$ is on the relative interior of the segment and $e$,
one of the locally longest edges incident to $p$,
  is perpendicular to the segment. We observe that moving $p$ in any direction
  would lengthen $e$.
%
\item[Type~3] Point $p$ is on the relative interior of the segment but not of Type $2$.
  Then there are two locally longest edges incident to $p$ laying in different half-planes delimited by a
  line perpendicular to the segment passing through $p$. We observe that moving $p$ in any direction would increase the length of one of these two edges.
\end{description}
%
Notably, if we know for any point $p$ on a segment that it is of  Type $1$ or $2$ and what its locally longest incident edge $e$ is, then we can deduce $p$'s position on the segment without any knowledge of other incident edges of $p$, just by minimizing the length of $e$.
%
Similarly, if we know that for any point $p$ on a segment that it  is of Type $3$ and what its pair of locally longest  incident edges $e,f$ is, then we can deduce $p$'s position on the segment without any knowledge of other incident edges of $p$, just by minimizing the length of $e$ and $f$.



\subsubsection*{Critical Paths}
Let $(E_1,\ldots,E_m)$ denote a  sequence of fixed points and segments, where $E_1$ and $E_m$ are fixed points or segments, and $E_2,\ldots,$ $E_{m-1}$ are segments.
%
A {\em critical path supported by} $(E_1,\ldots, E_m)$ consists of
points $p_1,\ldots, p_m$, where each $p_i$ is located at a selected
position on segment $E_i$. The $p_i$s are connected by edges $e_i$
such that (1) the edges are all of identical length, and (2) no
different selection of point locations on these segments results in a
sequence where no edge is longer but some edge is strictly shorter.
We may specify that the edges are of length $\lambda$ by writing
\emph{$\lambda$-critical path}.
%

%
Critical paths are useful in constructing minimum solution trees. Our algorithm makes use of the fact that it is possible to reduce the construction of  a minimum solution tree to computing a set of critical paths.
%

%
We will show below
(1) that a sequence $(E_1, \ldots, E_m)$ supports at most one critical path (under the assumption of general position) and
(2) how to compute a critical path supported by $(E_1, \ldots,$ $E_m)$---in case of existence---for a given precision $\delta$.
%

We introduce terminology that will aid us for both purposes. Given a sequence $(E_1,\ldots,E_m)$ and a positive number $\lambda$, let $U_i(\lambda)$ be the area around $E_i$ that can be reached from $E_1$ via $E_2, \ldots, E_{i-1}$ by edges of length at most $\lambda$. More exactly, let
%
\begin{itemize}
\item $U_1(\lambda)$ be the set of points in
the plane reachable from $E_1$ by an edge of length at most $\lambda$, and
\item $U_i(\lambda)$, $i>1$, be the set of points on the plane reachable
from $U_{i-1}(\lambda) \cap E_i$ by an edge of length at most $\lambda$.
\end{itemize}
%

Let $S_i(\lambda)$ be the set of points on the plane reachable from
$E_i$ by an edge of length exactly $\lambda$, such that
$p\in S_i(\lambda)$ implies that there is a $\lambda$-critical path $p_1,p_2,\ldots, p_i,p$ supported by $(E_1,E_2,\ldots, E_i,\{p\})$,
with $p_i\in E_i$ (note that $p$ need not be in one of the uncertainty
regions).  In particular, $S_i(\lambda)$ is contained, for $i>1$, in
the set of points on the plane reachable from
$S_{i-1}(\lambda) \cap E_i$ by an edge of length exactly $\lambda$.
We characterise the set $S_i(\lambda)$ more directly in Lemma 3.
%ALEJANDRO: definition above improved.  definition below now redundant
% %
% \begin{itemize}
% \item $S_1(\lambda)$ is the set of points in
% the plane reachable from $E_1$ by an edge of length exactly $\lambda$,
% \item $S_i(\lambda)$ for $i>1$ is the set of points on the plane reachable
% from $S_{i-1}(\lambda) \cap E_i$ by an edge of length exactly $\lambda$, and
% \item $e_1, \dots, e_{i-1}, e_i$ form a critical path, where $e_i$ is an edge of length $\lambda$ with one endpoint on $E_{i}$ and the other one can be chosen freely as long as the other conditions are satisfied.
% \end{itemize}


We study the properties of $U_i(\lambda)$ and $S_i(\lambda)$. By definition, $E_1$ consists of either a single point or a segment (Figure \ref{fig:e1}).
Further, $U_1(\lambda)$ consists either of a circle of radius $\lambda$ (Figure \ref{fig:e1}) or the Minkowski sum of a circle of radius $\lambda$ and a segment, and therefore also $U_1(\lambda) \cap E_2$---if not empty---consists of either a point or a subsegment of $E_2$.

\begin{figure}[h]
\begin{center}
\input{figureAlgorithmBa.tex}%
\hspace{2cm}
\input{figureAlgorithmBb.tex}%
\end{center}
\caption{Examples of $U_1(\lambda)$ and $S_1(\lambda)$ for the cases that $E_1$ is a fixed point (left)
and a segment (right).}
\label{fig:e1}
\hspace{0.05cm}
\end{figure}

In general we can deduce inductively the following lemma.

\begin{lemma}\label{lem:basic}
For $1< i \leq m$, if $U_{i-1}(\lambda) \cap E_i \not= \emptyset$ then $U_{i-1}(\lambda) \cap E_i$ consists of either  a single point of $E_i$ or a subsegment of $E_i$.
\end{lemma}

Using the definitions of $U_i(\lambda)$ and $S_i(\lambda)$, we have the following observation.

\begin{lemma}\label{lem:boundary}\label{subsec:l5}
For all $i \geq 1$, $S_i(\lambda)$ $\subseteq$ boundary of $U_i(\lambda)$.
\end{lemma}

\begin{proof} For $i=1$, it follows easily from the definition that
  $S_1(\lambda)$ is contained in the boundary of $U_1(\lambda)$.  
  Let $B$ be an open ball contained in $U_i(\lambda)$, with $p\in B$; we   
  will show that $p$ cannot be in $S_i(\lambda)$, and hence $S_i(\lambda)$ 
  can only contain boundary points.  For
  any $p'\in B$, since $B \subset U_i(\lambda)$, there is a path on 
  points $(p_1,p_2,\ldots, p_i,p')$,
  with $p_j\in E_j$, for $1\le j\le i$, with no edge longer than
  $\lambda$.  On the other hand, since $B$ is an open set, there exists a $p'\in B$ such that $\|p_ip\|<\|p_ip'\|$, for all choices of $p_i$ in $E_i$, and hence there exists a path on points
  $(p_1,p_2,\ldots, p_i,p')$ where
  $\|p_ip\|< \|p_ip'\|\le \lambda$.  Thus we have points $(p_1,p_2,\ldots, p_i,p)$ with  $\|p_jp_{j+1}\|\le \lambda$, for $1\le j<i$, and $\|p_ip\|<\lambda$ implying that $(E_1,E_2,\ldots, E_i,\{p\})$ does not support a $\lambda$-critical path, and therefore $p\not\in S_i(\lambda)$. $\Box$
  % This implies that
  % $p\not\in S_i(\lambda)$, since the edge $\|p_ip\|$ cannot be exactly of length $\lambda$ if $\|p_ip\|< \|p_ip'\|$. $\Box$
% %
%  To show that $S_i(\lambda)$ is a subset of the boundary of $U_i(\lambda)$
% for all $i>1$, it is sufficient to prove that any open set that contains a point of $S_i(\lambda)$ is not contained in the interior of  $U_i(\lambda)$. This can be shown by contradiction.
% If the open set is contained in the interior of $U_i(\lambda)$, the edge $e_i$ could be shortened, contradicting the critical path assumption that no edge in a critical path
% can be shortened without lengthening another. $\Box$.
% %
\end{proof}



\noindent We can conclude from the above lemma that, if $U_{i-1}(\lambda) \cap E_i = \emptyset$ then $S_{i-1}(\lambda) \cap E_i =\emptyset$.
%
Further, if $U_{i-1}(\lambda) \cap E_i$ consists of a single point $p$, then either $S_{i-1}(\lambda) \cap E_i = \emptyset$ or $S_{i-1}(\lambda) \cap E_i = \{p\}$.
%
If $U_{i-1}(\lambda) \cap E_i$ is a subsegment of $E_i$, then $S_{i-1}(\lambda) \cap E_i$ can be empty, consist of one or both extremities of the subsegment.
%, or is identical to the complete subsegment.
 %
In fact, we can prove the following lemma that describes $S_i(\lambda)$ more directly.

\begin{lemma}\label{subsec:l6}
\begin{enumerate}
  %(a)
  \item The set $S_1(\lambda)$ is the boundary of $U_1(\lambda)$.
  %(b)
  \item For all $i>1$, the set $S_i(\lambda)$ is the intersection of the boundary of $U_i(\lambda)$ with the Minkowski sum of a circle of radius $\lambda $ and $S_{i-1}(\lambda)\cap E_i$.
  \end{enumerate}
\end{lemma}

\begin{proof}\
\begin{enumerate}
%  (a)
  \item This fact follows from the definition of $S_1(\lambda)$ and ${U_1(\lambda)}$.
% (b)
 \item
  $\subseteq$: We make two observations. (1) By definition, $S_i(\lambda) \subseteq \{$points at distance exactly $\lambda$ from $S_{i-1}(\lambda) \cap E_i\}$. This set, in turn, is contained in the Minkowski sum of a circle of radius $\lambda$ and $S_{i-1}(\lambda)\cap E_i$. (2) From Lemma~\ref{lem:boundary}, we know that
  $S_i(\lambda)$ $\subseteq$ boundary of  $U_i(\lambda)$. Combining (1) and (2) gives us the result.


  $\supseteq$: Proof by Induction.  Let $p$ be any point in the
  intersection of the boundary of $U_i(\lambda)$ with the Minkowski
  sum of a circle of radius $\lambda $ and $S_{i-1}(\lambda)\cap E_i$.
  Then by definition there exists $q\in S_{i-1}(\lambda)\cap E_i$ and
  points $q_1,q_2,\ldots, q_{i-1}$ such that $\|qp\|=\lambda$ and the
  path $Q=(q_1,q_2, \ldots, q_{i-1},q)$ is a $\lambda$-critical path
  supported by $(E_1,E_2,\ldots, E_{i-1},\{q\})$.

  % We must show that for any choice of points

  % The edges of the path $q_1,q_2, \ldots, q_{i-1},q,p$ are
  % all of length exactly $\lambda$, it remains to be shown that
  % $q_1,q_2, \ldots, q_{i-1},q,p$ is a critical path supported by
  % $(E_1,E_2,\ldots, E_{i-1},E_i,\{p\})$, with edges of length exactly
  % $\lambda$.

  Suppose that $p\not\in S_i(\lambda)$.  This implies that
  $(E_1, E_2,\ldots, E_{i-1}, E_i, \{p\})$ does not support a
  $\lambda$-critical path.  In particular no edge of
  $(p_1, p_2, \ldots, p_{i-1}, p_i, p)$ is longer than $\lambda$, but
  some edge is strictly shorter, for some choice of points
  $p_j\in E_j$, for $1\le j \le i$; in particular, we have $\|p_ip\|\le \lambda$. On the other hand, we also have $\|p_ip\|\ge \lambda$,
  since $p$ is in the boundary of $U_i(\lambda)$, so by assumption,
  $\|p_ip\|=\lambda$.  If one of the edges in
  $(p_1, p_2, \ldots, p_{i-1}, p_i)$ is shorter than $\lambda$, then
  $p_i\in E_{i}(\lambda)\setminus S_{i-1}(\lambda)$, by definition of
  $S_{i-1}(\lambda)$.  On the other hand, there is exactly one point
  in $E_i$ that is distance $\lambda$ from $p$, and thus the
  existence of $p$ and $\|p_ip\|=\lambda$ imply that $p_i=q$, and therefore
  $p_i\in S_{i-1}\cap E_{i}$.  This is a contradiction, and therefore 
  % $(p_1,p_2, \ldots, p_{i-1},p_i,p)$ is a $\lambda$-critical path
  % supported by $(E_1,E_2,\ldots, E_{i-1},E_i,\{p\})$
  $p\in S_i(\lambda)$, as required.

%   % Now, since $p_i\in S_{i-1}(\lambda)$, there is
%   % no choice of points for $p_j$ in $E_j$, for $1\le j <E_{i-1}$ such
%   % that
% %  $q_1,q_2,\ldtos, q_{i-1},q$ 
%   $(p_1,p_2, \ldots, p_{i-1},p_i)$ has no edge longer than $\lambda$,
%   but at least one edge strictly shorter.  Since $p$ is in the
%   boundary of $U_i(\lambda)$, $p_ip$ has length at least $\lambda$.
%   Since $p$ is in the Minkowski sum of a circle of radius $\lambda$
%   and $S_{i-1}(\lambda)\cap E_i$, and $p_ip$ has length at least
%   $\lambda$, then the point $p_i$ is unique (for each $p$ in the set
%   $A$ [DEFINE A]), and thus $p_i\in S_{i-1}(\lambda \cap E_i$.... done.

%   then $p_ip$ has length at most
%   $\lambda$ [can't assume $p_i \in S_{i-1}(\lambda)$].
  
  
%   the path $Q$ is critical, we need only
%   consider perturbing $q$ on $E_i$, to make the edge $qp$ shorter than
%   lambda.

%   there is a path of edges of length $\lambda$ from $q$, which
%   we extend to $p$ by edge $e_i$.
%   We prove that  there is no other path to $p$ that uses edges that are all no longer than $\lambda$, but some are shorter. We show this by contradiction.
%   %
%   Suppose there is a choice of points $p_1,\ldots,p_i$ such that $p_1,\ldots,p_i,p$ is such a path. 
%   Suppose further that the last edge, $p_ip$, is shorter than $\lambda$. 
%   %
%   We know that $p_i, q \in U_i(\lambda)\cap E_i$. Further, $p$ is on the boundary of $U_i(\lambda)$, which means that the distance from $p_i$ to $p$
%   that is shorter than $\lambda$ is in contradiction to the definition of $U_i(\lambda)$. Thus, we know that the last edge in the path must be of length $\lambda$. Further, every other point from  $U_i(\lambda)\cap E_i$ must have a distance larger than $\lambda$ from $p$.  
  $\Box$


  \end{enumerate}
 \end{proof}


%%%%%%%%%%%TILL HERE%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent We deduce that the following cases for $S_i(\lambda)$ are possible (see Figure \ref{fig:stype}, depicting possibilities for $S_2(\lambda)$ for the case that $E_1$ is a fixed point).

\renewcommand{\redcolour}{darkgray}

\begin{figure}[h]
%
\centerline{
\input{figureAlgorithmDa.tex}
\hspace{0.65cm}
\input{figureAlgorithmDb.tex}
\hspace{0.65cm}
\input{figureAlgorithmDc.tex}
\hspace{0.65cm}
\input{figureAlgorithmDd.tex}
}
%
\caption{Shapes of $S_2(\lambda)$ of Type a, b, c, and d,
  respectively. $S_1(\lambda)$ is indicated with a dashed line,
  $S_1(\lambda) \cap E_2$ with open dots, and $S_2(\lambda)$ with dark
  gray curves.}
\label{fig:stype}
\end{figure}


\begin{description}
  \item[Type a.] $S_{i-1}(\lambda)\cap E_i = \emptyset$ and therefore $S_i(\lambda) = \emptyset$.
  \item[Type b.] $U_{i-1}(\lambda)\cap E_i$ consists of a single point $p$ and $S_{i-1}(\lambda)\cap
    E_i = \{p\}$. Then $S_i(\lambda)$ is a circle of
    radius $\lambda$ centered around $p$.
  \item[Type c.] $U_{i-1}(\lambda)\cap E_i$ is a subsegment of $E_i$ and
    $S_{i-1}(\lambda)\cap E_i$ is a single extremity of the subsegment. In
    this case, $U_i(\lambda)$ is the Minkowski sum of the subsegment and a ball
    of radius $\lambda$, and $S_i(\lambda)$ is the half circle of radius $\lambda$ centered
    on $S_{i-1}(\lambda)\cap E_i$ on the boundary of $U_i(\lambda)$.
   \item[Type d.] $U_{i-1}(\lambda)\cap E_i$ is a subsegment of $E_i$ and
    $S_{i-1}(\lambda)\cap E_i$ consists of both extremities of the
    subsegment. In this case, $U_i(\lambda)$ is the Minkowski sum of the
    subsegment and a ball of radius $\lambda$, and $S_i(\lambda)$ consists of both
    half circles of radius $\lambda$ each centered on a point of
    $S_{i-1}(\lambda)\cap E_i$ on the boundary of $U_i(\lambda)$.
\end{description}

\noindent For a given $(E_1,\ldots,E_m)$ and length $\lambda$ it is
therefore possible to compute successively the $U_i(\lambda)$'s and $S_i(\lambda)$'s. With this knowledge in hand, we are now ready to describe the computation of critical paths. The following lemma is crucial towards this goal.

\begin{lemma}\label{lem:critical}
A critical path exists for a sequence $(E_1,\ldots, E_m)$ if and only if there exists a $\lambda^* $ such that $U_{m-1}(\lambda^*) \cap E_m = S_{m-1}(\lambda^*) \cap E_m \neq \emptyset$. Furthermore, such a $\lambda^*$ is the smallest $\lambda$ such that $U_{m-1}(\lambda) \cap E_m \not= \emptyset$.
\end{lemma}
\begin{proof}
Figure~\ref{fig:em} illustrates the proof idea by describing types of possible outcomes for any $\lambda$ for the case of a sequence $(E_1, E_2, E_3)$ with $E_1$ a fixed point, for which $U_{2}(\lambda) \cap E_3$ is not empty.
%
\begin{figure}[h]
%
\centerline{
\input{figureAlgorithmEa.tex}
\hspace{0.75cm}
\input{figureAlgorithmEb.tex}
\hspace{0.75cm}
\input{figureAlgorithmEc.tex}
%\hspace{0.6cm}
%\input{figureAlgorithmEd.tex}
}

%
\caption{Sequence $(E_1,E_2,E_3)$ with outcomes of Type $\alpha$,
  $\beta$, and $\gamma$ respectively for the case that
  $U_2(\lambda) \cap E_3\not= \emptyset$.  $S_1(\lambda)$ is depicted
  by dashed lines, $S_1(\lambda) \cap E_2$ and $S_2(\lambda) \cap E_3$
  by open dots, and $S_2(\lambda)$ in dark gray.}
\label{fig:em}
\end{figure}
%
In general for any sequence $(E_1, \dots, E_m)$ the following shapes of $S_m(\lambda)$ are possible. Recall our general position assumption that no two lines are parallel. Using Lemma~\ref{lem:basic}, if $U_{m-1}(\lambda) \cap E_m \not= \emptyset$, either $U_{m-1}(\lambda) \cap E_m$ is a subsegment  of $E_m$ (Type $\alpha$ below) or it is a single point of $E_m$ (Type $\beta$ and $\gamma$ below).
\begin{description}
\item[Type $\alpha$.] If $E_m$ intersects the interior of $U_{m-1}(\lambda)$ then there is
  no $\lambda$-critical path. % of length $\lambda$. %ALEJANDRO: introduced notation
  A path with edges of length exactly $\lambda$ will not be critical as it can be shortened by moving the point location on $E_m$. %This case is shown in first part of Figure~\ref{fig:em} above.
\item[Type $\beta$.] If $U_{m-1}(\lambda) \cap E_m = S_{m-1}(\lambda) \cap E_m = \{p\}$ then there is a $\lambda$-critical path %of length $\lambda$
  as moving the point location
on $E_m$ only increases the edge length.  %This case is shown in the second part of Figure~\ref{fig:em} above.
\item[Type $\gamma$.] If $U_{m-1}(\lambda) \cap E_m$ is a single point and $S_{m-1}(\lambda) \cap E_m=\emptyset$,  there is no $\lambda$-critical path. %of length $\lambda$.
  In this case, moving the point location on $E_{m-1}$ gives a path with shorter edge length.%This is shown in the third part of Figure~\ref{fig:em} above.
%\item[Type $\delta$.] If $U_{m-1}(\lambda) \cap E_m$ is a segment and $S_{m-1}(\lambda) \cap
 % E_m$ is empty or consists only of extremities of the segment then there is no critical path of length $\lambda$.
\end{description}
To summarize, we observe that a critical path only exists for outcomes of Type $\beta$, and that this is the only outcome for which the condition given in the lemma is satisfied. Moreover, the $\lambda^*$ in outcomes of Type $\beta$ is the smallest value of $\lambda$ for which  $U_{m-1}(\lambda) \cap E_m \not= \emptyset$ since $U_{m-1}(\lambda) \cap E_m$ is a single point and decreasing the value of $\lambda$ any further will make it empty. $\Box$
\end{proof}


\newcommand{\caseone}{c.4}
\newcommand{\casetwo}{c.3}
\newcommand{\casethree}{c.2}
\newcommand{\casefoura}{c.1a}
\newcommand{\casefourb}{c.1b}
\newcommand{\casefive}{c.5}
\newcommand{\casesix}{c.6}
\newcommand{\pone}{\ensuremath{p_\ell}}
\newcommand{\ptwo}{\ensuremath{p_r}}
\newcommand{\fpone}{\ensuremath{f_{\pone}}}
\newcommand{\fptwo}{\ensuremath{f_{\ptwo}}}

Given $(E_1,\ldots, E_m)$, the following algorithm determines whether  $(E_1,\ldots, E_m)$ supports a critical path or not. If it does, the algorithm outputs the length of the edges in the critical path with a precision $\delta'$. Note that the need for a precision parameter arises only due to the algebraic nature of the problem since our computation involves binary search over real values. $\delta'$ is chosen depending on the precision bound, $\delta$, specified by the user and the input instance so that the loss in precision over all the steps of the algorithm is below the bound $\delta$. More precisely, we will choose $\delta' = \delta/k$.  We describe the reason for this choice after describing our algorithm. 

\begin{enumerate}
\item
Initialize $\lambda_{\min}$ and $\lambda_{\max}$ to be the minimum and the maximum distance between any adjacent pair $(E_i, E_{i+1})$ in the input sequence. Initialize
$\lambda$ to be $(\lambda_{\min}+\lambda_{\max})/2$.
\item
While ($\lambda_{\max}- \lambda_{\min} > \delta')$ do\\
\begin{itemize}
\item Compute $U_{m-1}(\lambda)$.
\item If $U_{m-1}(\lambda) \cap E_m = \emptyset$, then set $\lambda_{\min}$ to $\lambda$, set $\lambda$ to $(\lambda_{\min}+\lambda_{\max})/2$ and go to (2).
\item If $U_{m-1}(\lambda)\cap E_m \not= \emptyset$, then set  $\lambda_{\max}$ to $\lambda$, set $\lambda$ to $(\lambda_{\min}+\lambda_{\max})/2$ and go to (2).
\end{itemize}
\item
Check if $U_{m-1}(\lambda_{\max}) \cap E_m = S_{m-1}(\lambda_{\max}) \cap E_m \neq \emptyset$ up to perturbation $\delta'$ as explained below. If so, output $\lambda_{\max}$ as the edge-length of the critical path. If not, output that no critical path exists.
\end{enumerate}

We now give more details about the last step of our algorithm when the
shape of $S_{m-1}(\lambda_{\max})$ is of Type d and $m\ge 3$; that is,
where $S_{m-2}(\lambda_{\max}) \cap E_{m-1}$, for $m\ge 3$, comprises
exactly two distinct points, denoted $\pone$ and $\ptwo$.  This
procedure is similar to what is needed to handle other non-trivial
shapes of $S_{m-1}(\lambda_{\max})$, i.e., Types $b$ and $c$ as well
as $S_1(\lambda_{\max})$, when $m=2$. We will denote
$U_{m-1}(\lambda_{\max}) \cap E_m$ by $L$ if it is a line segment and
by $q$ if it is a point. For a point $p\in \{\pone,\ptwo\}$ and a line
segment $L$, let $f_p$ denote the point on $L$ closest to point
$p$. The algorithm will detect if one of the six (mutually exclusive)
cases described in Figure~\ref{fig:detect-type-beta} occurs, where we
assume that in all cases the segment $\pone\ptwo$ does not intersect
$E_m$. Procedures for this detection can be easily derived from high
level descriptions\footnote{The descriptions are evident from
  Figure~\ref{fig:detect-type-beta}, except perhaps the difference
  between c.1b and c.2.  These are distinguished by the fact that
  $\fptwo$ lies outside the semi-disc for c.1b, and inside the
  semi-disc for c.2, where $p$ is $\pone$ or $\ptwo$, as appropriate.}
of the cases. In each case the algorithm performs a test, as follows:

\begin{description}
\item[Case 1a and 1b:] Test if the length of line segment $L$ is at
  most $\delta'$.
\item[Cases 2-4:] Test if $\lambda_{\max} - d(p,f_p)$ is at most $\delta'$. Here, $p$ will be either $\pone$ or $\ptwo$ depending on which semicircle is intersected by $L$.
\item[Case 5:] Test if the minimum distance from $q$ to either semicircle is at most $\delta'$.
\item[Case 6:] Test if $\lambda_{\max} - d(p,f_p)$ is at most
  $\delta'$. Here, $p$ will be either $\pone$ or $\ptwo$ depending on
  which is closer to $L$ (Note that by the general position assumption,
  one of them will be closer).
\end{description}

If one of the above cases occurs and its test returns true, there is
a $\lambda^* \in [\lambda_{\min}, \lambda_{\max}]$  of Type
$\beta$, as illustrated in Figure~\ref{fig:em}, and hence a critical
path exists. For the two other possible scenarios (Type $\alpha$ and
Type $\gamma$) either none of cases 1-6 occur or the corresponding
test fails, and the algorithm concludes that the critical path does
not exist. These cases are also illustrated in Figure~\ref{fig:em}.


\def\svgwidth{0.8\textwidth}
\begin{figure}[h]
  \centering
  \input{type-beta-detection.eps_tex}
  \caption{Cases 1-6 where we test for for $\lambda^*$ of Type-$\beta$
    (up to perturbation $\delta'$).  Each line segment labelled $c.i$,
    for $1\le i \le 6$, represents a possible instance of $E_{m}$.}
  \label{fig:detect-type-beta}
\end{figure}

As a consequence of Lemma~\ref{lem:critical}, we have the following
corollary. It will help us convert a set of line segments, for which
we have found a critical path, into a set of fixed points, resulting
in an input with fewer line segments.

\begin{corollary}
  \label{cor:critical}
  If  $(E_1,\ldots,E_m)$ supports a critical path consisting of edges that are locally longest in a minimum solution tree, then there is a unique choice of point locations that defines the critical path. Furthermore, this choice of point locations is a part of the optimal solution.
\end{corollary}

%{\bf This corollary likely deserves a proof.}

\subsubsection*{Description of the Algorithm}

We now show how to compute a best point set
by examining all possible critical paths.

%\newcommand{\ems}{\ensuremath{}}

Note that if we had an oracle giving us a sequence $(E_1,E_2,\ldots,
E_m)$ that supports a critical path consisting of edges that are
locally longest in the best point set, then we could determine the
choice of points on $(E_1,E_2,\ldots, E_m)$ these elements in the best
point set. We could then replace the segments in the sequence by fixed
points and solve the rest of the problem separately.  This eventually
would allow us to replace all segments by fixed points, and then to
solve the problem by finding an associated MBST.  Lacking an oracle we
determine these sequences \emph{by complete enumeration} of \emph{all
  possible sequences} $(E_1,E_2,\ldots,E_m)$ that contain at least one
segment, where $E_1$ and $E_m$ are fixed points or segments, and
$E_2,E_3,\ldots,E_{m-1}$ are segments.  There are $O(n^2 \cdot k!
\cdot k)$ such sequences\footnote{Count the number of ordered
  $i$-subsets of $k$ segments by $\sum_{i=1}^k k!/(k-i)!$, and
  multiply these by the $(n^2+n+1)$ to count ways that $E_1$ and $E_m$
  might be points.}.  This enumeration accounts for most of the
complexity of our recursive algorithm, in which we initialize $b$ to
$\infty$ at the top level call, and proceed as follows:
\begin{enumerate}
\item If the instance does not contain any segments, we compute an MST
  with a greedy algorithm, in polynomial time, and report the length
  $b'$ of the bottleneck edge.
\item Else, for each sequence in the enumeration, if it supports an
  $\ell$-critical path, for some $\ell$, do the following: 
  \begin{enumerate}
  \item If $\ell> b$, do nothing; that is, we prune these sequences in
    the enumeration as we find them.  
  \item Else, if $\ell \le b$, we replace the segments of the sequence
    with the unique fixed points defined by the $\ell$-critical path
    and recurse on the updated set of sequences and points, with $b$
    (in the recursive call only) initialized to $\ell$.  Let $b'$ be
    the output of the recursive call.  
  \item If $b'< b$, set $b$ to $b'$.
  \end{enumerate}
\item If no MST is found, report $\infty$, else report $b$.
\end{enumerate}



% Once we have gone through the
% complete list of possible sequences, we will have found the best
% critical path with edges that are locally longest in a minimum
% solution tree.  

% The main steps of our algorithm can be summarized as follows:
% \begin{enumerate}
% \item Enumerate all possible sequences of the form $(E_1,\ldots,E_m)$,
%   where $E_1$ and $E_m$ are fixed points or segments, and
%   $E_2,\ldots,E_{m-1}$ are segments.
% \item For each such sequence:
%   \begin{enumerate}
%   \item check if it supports a critical path and if so, compute the
%     edge-length $\ell$ of the critical path and the choice of point
%     locations in the path.
% \item If $\ell$ is at most some number... do stuff

%   While the current (possibly partial) solution improves the
%   previous best known solution, run the algorithm recursively on the
%   reduced instance obtained by fixing the points locations on the
%   critical path.  Look only for critical paths of edge-lengths at most
%   $\ell$ and abort if no such path is found.

%   \end{enumerate}
% \item Continue until no line segments remain. Compute the MST on the
%   resulting set of points using the greedy algorithm.  Update if the
%   new MST is preferred over the previous best MST.
% \end{enumerate}


We remark that it is crucial to compute critical paths with
progressively decreasing edge lengths since positions of points on
segments are determined by locally longest edges incident to them;
this is enforced in recursive calls with the parameter $b$.
Furthermore, updating $b$ in step 2(c) allows us to prune the search
in step 2(a) by discarding critical paths whose longest edge is too
long.  Finally, the algorithm terminates because we only enumerate
sequences with at least one segment.

We show by induction on $k$ that the algorithm correctly outputs the
length of the bottleneck edge of a minimum solution tree.  The
algorithm is correct when there are $0$ segments.  Suppose it is
correct for up to $k-1$ segments.  If we call the algorithm with $k$
segments, for $k>0$, then at least one of the sequences
$(E_1,E_2,\ldots, E_m)$ supports an $\ell$-critical path whose edges
are not only locally longest in a minimum solution tree, but also
globally longest among sequences of critical paths supported by at
least one segment.  Thus the sequence satisfies the antecedents of
Corollary~\ref{cor:critical}, and furthermore, all other critical
paths in the minimum solution tree will be found in the recursive
calls. By the inductive hypothesis, the recursive call returns the
length of the bottleneck edge $b'$ of a minimum solution tree on the
reduced input, and by Corollary~\ref{cor:critical} this is also the
length of a bottleneck edge on the unreduced input (we may have $b'>
\ell$, however). We have shown that for $k$ segments the output is at
most the length of a bottleneck edge of a minimum solution tree on the
input points and segments; on the other hand, the output value cannot
be smaller than this, since the value is, in any case, derived from
the bottleneck edge of an MST on a set of points chosen from the $n+k$
input regions.

With regards to precision, when we replace the line segments with
fixed points, our choice is correct within $\delta'$ of the true
value.  Since our algorithm is recursive, this choice of points will in
turn influence the choice of points in the next round of
recursion. Since our algorithm is computing distances between points,
the edge lengths of the critical path computed in level $i$ of the
recursion will be correct up to a precision of $i\delta’$ (using the
triangle inequality). Since the last level of recursion, level $k$,
requires a precision of $\delta$, we will fix $k\delta' = \delta$ in
our analysis.



The enumeration in our algorithm described above is superexponential in the number $k$ of segments,
which is not surprising since we have shown the problem with no fixed points is
NP-hard.  For constant $k$ the problem is, however, polynomial in the number $n$ of points, as our running time analysis will show.

The (multiple recursive) enumeration results in a search tree of size $O((n^2 \cdot k! \cdot k)^k)$  with an $O(k)$ running time for each node in the search tree. Thus the total time complexity is
$O((n^2 \cdot k! \cdot k)^k \cdot k)$.

\begin{theorem}
  The BCU problem for a set of $n$ fixed points and $k$ line segments
  can be solved in time $O((n^2 \cdot k! \cdot k)^k \cdot k)$, for any
  fixed precision $\delta$.
\end{theorem}


==> clauseGadgetPoints.tex <==
\begin{figure}[h]
\begin{center}
 \psset{unit=1.3cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
 \pspicture(0,2)(8,8.5)
 %
 \dotnode(1,1.5){a0}
 \dotnode(4,8.5){a1}
 \dotnode(7,1.5){a2}
 %
 \dotnode[linewidth=1.5pt,linecolor=gray](1,3){a3}
 \dotnode(2,2.5){a4}
 \dotnode(2,3.5){a5}
 \dotnode(2.5,3.5){aa5}
 \dotnode(3,3.5){a6}
 \dotnode(3.5,3.5){aa6}
 \dotnode(4,4){a7}
 \dotnode(3,7){a8}
 \dotnode(4.5,3.5){aa7}
 \dotnode(5,3.5){a9}
 \dotnode(5.5,3.5){aa8}
 \dotnode(6,3.5){a10}
 \dotnode[linewidth=1.5pt,linecolor=gray](7,3){a11}
 \dotnode(8,2.5){a12}
 \dotnode(8,3.5){a13}
 \dotnode(8,4.5){a14}
 \dotnode(8,5.5){a15}
 \dotnode(8,6.5){a16}
 \dotnode(7.5,6.5){aa16}
 \dotnode(7,6.5){a17}
 \dotnode(6.5,6.5){aa17}
 \dotnode(6,6.5){a18}
 \dotnode(5.5,6.5){aa18}
 \dotnode(5,6.5){a19}
 \dotnode[linewidth=1.5pt,linecolor=black,dotstyle=o](4,6.5){a20}
 \dotnode(3,6.5){a21}
 \dotnode(2.5,6.5){aa21}
 \dotnode(2,6.5){a22}
 \dotnode(1.5,6.5){aa22}
 \dotnode(1,6.5){a23}
 \dotnode(0.5,6.5){aa23}
 \dotnode(0,6.5){a24}
 \dotnode(0,5.5){a25}
 \dotnode(0,4.5){a26}
 \dotnode(0,3.5){a27}

 \dotnode(1,2){b0}
 \dotnode(4,8){b1}
 \dotnode(7,2){b2}
 \dotnode[linewidth=1.5pt,linecolor=black,dotstyle=o](1,3.5){b3}
 \dotnode(2,3){b4}
 \dotnode(2,4){b5}
 \dotnode(2.5,4){bb5}
 \dotnode(3,4){b6}
 \dotnode(3.5,4){bb6}
 \dotnode(4,3.5){b7}
 \dotnode(4.5,4){bb7}
 \dotnode(3,7.5){b8}
 \dotnode(5.5,4){bb8}
 \dotnode(5,4){b9}
 \dotnode(6,4){b10}
 \dotnode[linewidth=1.5pt,linecolor=black,dotstyle=o](7,3.5){b11}
 \dotnode(8,3){b12}
 \dotnode(8,4){b13}
 \dotnode(8,5){b14}
 \dotnode(8,6){b15}
 \dotnode(8,7){b16}
 \dotnode(7.5,6){bb16}
 \dotnode(7,6){b17}
 \dotnode(6.5,6){bb17}
 \dotnode(6,6){b18}
 \dotnode(5.5,6){bb18}
 \dotnode(5,6){b19}
 \dotnode[linewidth=1.5pt,linecolor=gray](4,7){b20}
 \dotnode(3,6){b21}
 \dotnode(2.5,6){bb21}
 \dotnode(2,6){b22}
 \dotnode(1.5,6){bb22}
 \dotnode(1,6){b23}
 \dotnode(0.5,6){bb23}
 \dotnode(0,7){b24}
 \dotnode(0,6){b25}
 \dotnode(0,5){b26}
 \dotnode(0,4){b27}


 \psset{linecolor=black,nodesep=.1,linestyle=dashed}
 \ncline{a0}{b0}
 \ncline{a1}{b1}
 \ncline{a2}{b2}
 \ncline{a3}{b3}
 \ncline{a4}{b4}
 \ncline{a5}{b5}
 \ncline{a6}{b6}
 \ncline{a7}{b7}
 \ncline{a8}{b8}
 \ncline{a9}{b9}
 \ncline{a10}{b10}
 \ncline{a11}{b11}
 \ncline{a12}{b12}
 \ncline{a13}{b13}
 \ncline{a14}{b14}
 \ncline{a15}{b15}
 \ncline{a16}{b16}
 \ncline{a17}{b17}
 \ncline{a18}{b18}
 \ncline{a19}{b19}
 \ncline{a20}{b20}
 \ncline{a21}{b21}
 \ncline{a22}{b22}
 \ncline{a23}{b23}
 \ncline{a24}{b24}
 \ncline{a25}{b25}
 \ncline{a26}{b26}
 \ncline{a27}{b27}
 \ncline{aa5}{bb5}
 \ncline{aa6}{bb6}
 \ncline{aa7}{bb7}
 \ncline{aa8}{bb8}
 \ncline{aa16}{bb16}
 \ncline{aa17}{bb17}
 \ncline{aa18}{bb18}
 \ncline{aa21}{bb21}
 \ncline{aa22}{bb22}
 \ncline{aa23}{bb23}

 \psset{linecolor=gray,linestyle=solid,nodesep=0pt,arcangle=20,arrows=-}
 \ncarc{->}{a3}{b0}
 \ncarc{a3}{b4}
 \ncarc{b4}{a5}
 \ncarc{->}{b20}{b1}
 \ncarc{b20}{a8}
 \ncarc{a8}{a21}
 \ncarc{->}{a11}{b2}
 \ncarc{a11}{b12}
 \ncarc{b12}{a13}

 \psset{linecolor=black,linestyle=dashed}
 \ncarc{a27}{b3}
 \ncarc{b3}{a5}
 \ncarc{a10}{b11}
 \ncarc{b11}{a13}
 \ncarc{a20}{a19}
 \ncarc{a21}{a20}


 % \psset{linecolor=black,linestyle=solid}
 % \ncarc{a6}{a5}
 % \ncarc{b7}{a6}
 % \ncarc{a9}{b7}
 % \ncarc{a10}{a9}
 % \ncarc{a13}{a14}
 % \ncarc{a14}{a15}
 % \ncarc{a15}{a16}
 % \ncarc{a16}{a17}
 % \ncarc{a17}{a18}
 % \ncarc{a18}{a19}
 % \ncarc{a21}{a22}
 % \ncarc{a22}{a23}
 % \ncarc{a23}{a24}
 % \ncarc{a24}{a25}
 % \ncarc{a25}{a26}
 % \ncarc{a26}{a27}

  \psset{linecolor=black,linestyle=solid}
 \ncarc{a5}{aa5}
 \ncarc{aa5}{a6}
% \ncarc{a6}{a5}
 \ncarc{a6}{aa6}
 \ncarc{aa6}{b7}
% \ncarc{b7}{a6}
 \ncarc{b7}{aa7}
 \ncarc{aa7}{a9}
% \ncarc{a9}{b7}
 \ncarc{a9}{aa8}
 \ncarc{aa8}{a10}
% \ncarc{a10}{a9}
 \ncarc{a13}{a14}
 \ncarc{a14}{a15}
 \ncarc{a15}{a16}
 \ncarc{a16}{aa16}
 \ncarc{aa16}{a17}
% \ncarc{a16}{a17}
 \ncarc{a17}{aa17}
 \ncarc{aa17}{a18}
 % \ncarc{a17}{a18}
 \ncarc{a18}{aa18}
 \ncarc{aa18}{a19}
% \ncarc{a18}{a19}
 \ncarc{a21}{aa21}
 \ncarc{aa21}{a22}
 % \ncarc{a21}{a22}
 \ncarc{a22}{aa22}
 \ncarc{aa22}{a23}
% \ncarc{a22}{a23}
 \ncarc{a23}{aa23}
% \ncarc{a23}{a24}
 \ncarc{aa23}{a24}
 \ncarc{a24}{a25}
 \ncarc{a25}{a26}
 \ncarc{a26}{a27}

 \psframe[linearc=.25,linecolor=gray](2.9,5.9)(5.1, 8.6)
 
 \endpspicture
\end{center}
 \vspace*{10pt}
 \caption{An example clause gadget.  As shown, aside from vertical
   sequences of uncertainty pairs leading to variable gadgets, there
   are no other uncertainty pairs in the vicinity of the clause
   gadget.  The graph $G_1$ can be connected only if at least one of
   the gray points is chosen; that is, the attached literal is set to
   \true. The gate inside the gray box can be moved up one unit to
   meet variable-clause connectors at different heights, if
   necessary.}
\label{clause_gadget_points}
\end{figure}


==> clauseGadgetSquares.tex <==
\begin{figure}[h]
\begin{center}
 \psset{unit=0.3cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
 \pspicture(-6,3)(15,19)

 \psgrid[gridcolor=lightgray,subgriddiv=1,gridwidth=0.001pt,gridlabels=0pt](0,0)(-7,3)(16,19)

 \psline(0,4)(1,4)(1,5)(0,5)(0,4)
 \psline(0,9)(1,9)(1,10)(0,10)(0,9)
 \psline(14,18)(15,18)(15,19)(14,19)(14,18)
 \psline(9,18)(10,18)(10,19)(9,19)(9,18)
 \psline(-1,18)(0,18)(0,19)(-1,19)(-1,18)
 \psline(-6,18)(-5,18)(-5,19)(-6,19)(-6,18)
 \psline[linecolor=gray,linewidth=1.5pt](4,14)(5,14)(5,15)(4,15)(4,14)
 \psdots[linecolor=\bluecolour](1,5)(1,10)(4,14)
 \psdots[linecolor=\bluecolour,dotstyle=Bo](15,18)(10,18)
 \psdots[linecolor=\bluecolour,dotstyle=x](0,18)(-5,18)(4,15)

 \psdots[linecolor=\redcolour](1,4)(1,9)
 \psdots[linecolor=\redcolour,dotstyle=Bo](14,18)(9,18)(5,15)
 \psdots[linecolor=\redcolour,dotstyle=x](-1,18)(-6,18)

 \pnode(4,14){a1}
 \pnode(1,10){a2}
 \pnode(1,5){a3}
 \pnode(1.5,3){a4}


 \pnode(16.5,18){b0}
 \pnode(15,18){b1}
 \pnode(10,18){b2}


 \pnode(4,15){c1}
 \pnode(0,18){c2}
 \pnode(-5,18){c3}
 \pnode(-7,17.5){c4}


 \pnode(1,2.5){d0}
 \pnode(1,4){d1}
 \pnode(1,9){d2}


 \pnode(5,15){e1}
 \pnode(9,18){e2}
 \pnode(14,18){e3}
 \pnode(16,17.5){e4}


 \pnode(-7.5,18){f0}
 \pnode(-6,18){f1}
 \pnode(-1,18){f2}

 \psset{linecolor=\bluecolour}
 \ncline{->}{a1}{a2}
 \ncarc[arcangle=30]{->}{a2}{a3}
 \ncarc[arcangle=30]{->}{a3}{a4}
 \ncline{->}{c1}{c2}
 \ncarc[arcangle=30]{->}{c2}{c3}
 \ncarc[arcangle=30]{->}{c3}{c4}
 \ncarc[arcangle=30]{->}{b0}{b1}
 \ncarc[arcangle=30]{->}{b1}{b2}

 \psset{linecolor=\redcolour}
 \ncline{->}{e1}{e2}
 \ncarc[arcangle=-30]{->}{e2}{e3}
 \ncarc[arcangle=-30]{->}{e3}{e4}
 \ncarc[arcangle=-30]{->}{d0}{d1}
 \ncarc[arcangle=-30]{->}{d1}{d2}
 \ncarc[arcangle=-30]{->}{f0}{f1}
 \ncarc[arcangle=-30]{->}{f1}{f2}

 \psset{linecolor=black}

 %END NEW
%  \psline(0,4)(1,4)(1,5)(0,5)(0,4)
%  \psline(0,9)(1,9)(1,10)(0,10)(0,9)
%  \psline(14,18)(15,18)(15,19)(14,19)(14,18)
%  \psline(9,18)(10,18)(10,19)(9,19)(9,18)
%  \psline(-1,18)(0,18)(0,19)(-1,19)(-1,18)
%  \psline(-6,18)(-5,18)(-5,19)(-6,19)(-6,18)
%  \psline[linecolor=gray,linewidth=1.5pt](4,14)(5,14)(5,15)(4,15)(4,14)
%  \psdots[linecolor=\bluecolour,dotstyle=triangle*](1,5)(1,10)(4,14)
%  \psdots[linecolor=\bluecolour,dotstyle=square*](14,18)(9,18)(5,15)  \psdots[linecolor=\bluecolour,dotstyle=*](0,18)(-5,18)(4,15)

%  \psdots[linecolor=\redcolour,dotstyle=triangle*](1,4)(1,9)
%  \psdots[linecolor=\redcolour,dotstyle=square*](15,18)(10,18)
% \psdots[linecolor=\redcolour,dotstyle=*](-1,18)(-6,18)

%  \pnode(4,14){a1}
%  \pnode(1,10){a2}
%  \pnode(1,5){a3}
%  \pnode(1.5,3){a4}



%  \pnode(16.5,18){b0}
%  \pnode(15,18){b1}
%  \pnode(10,18){b2}


%  \pnode(4,15){c1}
%  \pnode(0,18){c2}
%  \pnode(-5,18){c3}
%  \pnode(-7,17.5){c4}


%  \pnode(1,2.5){d0}
%  \pnode(1,4){d1}
%  \pnode(1,9){d2}


%  \pnode(5,15){e1}
%  \pnode(9,18){e2}
%  \pnode(14,18){e3}
%  \pnode(16,17.5){e4}


%  \pnode(-7.5,18){f0}
%  \pnode(-6,18){f1}
%  \pnode(-1,18){f2}

 
%  \psset{linecolor=\bluecolour}
%  \ncline{->}{a1}{a2}
%  \ncarc[arcangle=30]{->}{a2}{a3}
%  \ncarc[arcangle=30]{->}{a3}{a4}
%  \ncline{->}{c1}{c2}
%  \ncarc[arcangle=30]{->}{c2}{c3}
%  \ncarc[arcangle=30]{->}{c3}{c4}
%  \ncline{->}{e1}{e2}
%  \ncarc[arcangle=-30]{->}{e2}{e3}
%  \ncarc[arcangle=-30]{->}{e3}{e4}

%  \psset{linecolor=\redcolour}
%  \ncarc[arcangle=-30]{->}{d0}{d1}
%  \ncarc[arcangle=-30]{->}{d1}{d2}
%  \ncarc[arcangle=-30]{->}{f0}{f1}
%  \ncarc[arcangle=-30]{->}{f1}{f2}
%  \ncarc[arcangle=30]{->}{b0}{b1}
%  \ncarc[arcangle=30]{->}{b1}{b2}

%  \psset{linecolor=black}

 \endpspicture
 \caption{An example clause gadget.  The \redcolour\ arrow connecting
   the core square to the top right arm represents a connection to a
   negated variable.}
\label{fig:clausegadget}
\end{center}
\end{figure}


==> conclusion.tex <==
\section{Conclusions}
\label{sec:other}

A number of open problems remain.
 It would be interesting to show NP-hardness results for the BCU problem for other uncertainty regions, such as disks.
%It will be nice to prove a similar result for other regions like disks.
It is also possible that techniques from convex optimization could be used to design approximation algorithms for BCU for, say, line segments or squares.
%From the perspective of fixed parameter tractability, we observed that
%BCU is in FPT when the instance consists of $n$ fixed points and $k$ pairs of points; the parameter is $k$. 
We conjecture that BCU for the case of line segments is W[1]-hard and hence our exact algorithm is unlikely to be improved upon significantly.

Although we have been
able to obtain several NP-hardness results for BCU, we do not have any
complexity lower bounds for WCU which, a priori, seems harder. It is an
interesting open question to improve our approximation algorithms for both
these problems.

In conclusion, our work on connectivity problems for uncertainty regions motivated by wireless network scenarios suggests that this area provides a rich collection of problems for further investigation.


%If we assume centers to be chosen, say, uniformly at random in a square, and points within the disks to again be chosen uniformly at random, can we say anything probabilistically about the average case?  We have shown that the ``cinch-up'' heuristic is a constant-factor approximation for the $B\alpha$ Problem for non-overlapping disks.  As the number of disks, $n$, approaches infinity we have a family of examples showing that it can be as bad as a $3/2$-approximation. Is there a heuristic that multiplicatively approaches OPT as $n \rightarrow \infty$, or at least does better than ``cinch-up''?

%What can we say about the average case $\alpha$ problem?  It seems intuitive that taking the center of disks and the associated maximum length edge of the associated BSpT should yield the average case $\alpha$ - but is this really the case?  Is this problem possible to analyze analytically?  If not amenable to direct analysis, it is at least easy enough to simulate, though we leave this for future work.

%Another interesting family of problems arises when we mandate that the regions be non-overlapping, as one might want to do in specifying regions in practice.  In this constrained problem we should be able to come up with improved estimates compared with those in Lemmas \ref{lemma:best_case_opt+1},  \ref{lemma:worst_case_opt+1} and \ref{lemma:worst_case_2*opt}. Moreover,  the construction of Lemma \ref{lemma:worst_case_lower_bound} is clearly no longer applicable.

%Another interesting direction to push the intractability results is for the case of few uncertainty regions.  It seems likely that one might encounter problems of the type first noticed by Bajaj \cite{b-pgans-86}, \cite{b-adgop-88} in trying to solve the Fermat-Weber problem (see also \cite{SCG06},  section 3.2.1 and appendix) in the best and worst-case $\alpha$ problems for square or disk shaped uncertainty regions even when $N$ is relatively small.


==> connectingGadgetsSquares.tex <==
\begin{figure}
\begin{center}
 \psset{unit=0.3cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
 \pspicture(4,-1)(15,8)

 \psgrid[gridcolor=lightgray,subgriddiv=1,gridwidth=0.001pt,gridlabels=0pt](0,0)(4,-1)(15,8)

 \psline(4,0)(5,0)(5,1)(4,1)(4,0)
 \psline(9,0)(10,0)(10,1)(9,1)(9,0)
 \psline(14,0)(15,0)(15,1)(14,1)(14,0)

 \psline(4,6)(5,6)(5,7)(4,7)(4,6)
 \psline(9,6)(10,6)(10,7)(9,7)(9,6)
 \psline(14,6)(15,6)(15,7)(14,7)(14,6)

 \psline(9,2)(10,2)(10,3)(9,3)(9,2)
 \psline(9,4)(10,4)(10,5)(9,5)(9,4)


 \psdots(9.5,2.5)(9.5,4.5)
 \psset{linecolor=\bluecolour}
 \pnode(2.5,1){a2}
 \dotnode(4,1){a3}
 \dotnode(9,1){a4}
 \dotnode(14,1){a5}
 \pnode(16,1.5){a55}
 \pnode(2.5,7){a59}
 \dotnode(4,7){a6}
 \dotnode(9,7){a7}
 \dotnode(14,7){a8}
 \pnode(16,7.5){a85}

 \ncarc[arcangle=30]{->}{a2}{a3}
 \ncarc[arcangle=30]{->}{a3}{a4}
 \ncarc[arcangle=30]{->}{a4}{a5}
 \ncarc[arcangle=30]{->}{a5}{a55}
 \ncarc[arcangle=30]{->}{a59}{a6}
 \ncarc[arcangle=30]{->}{a6}{a7}
 \ncarc[arcangle=30]{->}{a7}{a8}
 \ncarc[arcangle=30]{->}{a8}{a85}

 \psset{linecolor=\redcolour}
 \pnode(3,1.5){b2}
 \dotnode(5,1){b3}
 \dotnode(10,1){b4}
 \dotnode(15,1){b5}
 \pnode(16.5,1){b55}
 \pnode(3,7.5){b59}
 \dotnode(5,7){b6}
 \dotnode(10,7){b7}
 \dotnode(15,7){b8}
 \pnode(16.5,7){b85}
 \ncarc[arcangle=30]{<-}{b2}{b3}
 \ncarc[arcangle=30]{<-}{b3}{b4}
 \ncarc[arcangle=30]{<-}{b4}{b5}
 \ncarc[arcangle=30]{<-}{b5}{b55}
 \ncarc[arcangle=30]{<-}{b59}{b6}
 \ncarc[arcangle=30]{<-}{b6}{b7}
 \ncarc[arcangle=30]{<-}{b7}{b8}
 \ncarc[arcangle=30]{<-}{b8}{b85}

 \psset{linecolor=black}
 \pnode(9.5,2.5){c1}
 \pnode(9.5,4.5){c2}

 \ncline[linestyle=dashed]{c1}{b4}
 \ncline[linestyle=dashed]{c1}{a4}
 \ncline[linestyle=dashed]{c1}{c2}
 \ncline[linestyle=dashed]{c2}{b7}
 \ncline[linestyle=dashed]{c2}{a7}

 \endpspicture
\caption{An example of a loose connection.}
\label{fig:forestlink}
\end{center}
\end{figure}


==> connector.tex <==
\begin{figure}[h]

\centering
\hspace*{2cm}
\begin{tabular}{ccc}

 \psset{unit=1.3cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
 \pspicture(-1,0)(1,5)

 \psset{linecolor=gray,linewidth=0.5pt}
 \dotnode(-2,0.5){a0}
 \dotnode(-2,1.5){a1}
 \dotnode(-2,2.5){a2}
 \dotnode(-2,3.5){a3}
 \dotnode(-2,4.5){a4}


 \psset{linecolor=black,linewidth=0.5pt}
 \dotnode(-2,1){b0}
 \dotnode(-2,2){b1}
 \dotnode(-2,3){b2}
 \dotnode(-2,4){b3}
 \dotnode(-2,5){b4}


 \psset{linecolor=black,nodesep=.1,linestyle=dashed}
 \ncline{a0}{b0}
 \ncline{a1}{b1}
 \ncline{a2}{b2}
 \ncline{a3}{b3}
 \ncline{a4}{b4}


 \psset{linecolor=gray,nodesep=0,arcangle=30,linestyle=solid,arrows=->}
 \ncarc{a0}{a1}
 \ncarc{a1}{a2}
 \ncarc{a2}{a3}
 \ncarc{a3}{a4}

 \psset{linecolor=black,arrows=->}
 \ncarc{b1}{b0}
 \ncarc{b2}{b1}
 \ncarc{b3}{b2}
 \ncarc{b4}{b3}

 \psset{linecolor=black,arrows=-}
 \endpspicture

&

\  \hspace*{2.5cm}

&

 \psset{unit=0.45cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=0.5pt}
 \pspicture(-1,-1)(5,14)

 \psset{linecolor=black,linewidth=0.5pt}
 \dotnode(0,1){b0}
 \dotnode(0,3){b1}
 \dotnode(0,5){b2}

 \psset{linecolor=black,dotstyle=o,linewidth=0.5pt}
 \dotnode(1,6){b3}

 \psset{linecolor=black,dotstyle=oplus,linewidth=0.5pt}
 \dotnode(2,5){b4}
 \dotnode(4,5){b5}
 \dotnode(4,7){b6}
 \dotnode(4,9){b7}
 \dotnode(2,9){b8}
 \dotnode(0,9){b9}
 \dotnode(0,11){b10}
 \dotnode(0,13){b11}

 \psset{linecolor=gray,dotstyle=*,linewidth=0.5pt}
 \dotnode(0,0){a0}
 \dotnode(0,2){a1}
 \dotnode(0,4){a2}

 \psset{linecolor=black,dotstyle=o,linewidth=0.5pt}
 \dotnode(1,5){a3}

 \psset{linecolor=black,dotstyle=otimes,linewidth=0.5pt}
 \dotnode(2,4){a4}
 \dotnode(4,4){a5}
 \dotnode(4,6){a6}
 \dotnode(4,8){a7}
 \dotnode(2,8){a8}
 \dotnode(0,8){a9}
 \dotnode(0,10){a10}
 \dotnode(0,12){a11}


 \psset{linecolor=black,dotstyle=*,nodesep=.1,linestyle=dashed}
 \ncline{a0}{b0}
 \ncline{a1}{b1}
 \ncline{a2}{b2}
 \ncline{a3}{b3}
 \ncline{a4}{b4}
 \ncline{a5}{b5}
 \ncline{a6}{b6}
 \ncline{a7}{b7}
 \ncline{a8}{b8}
 \ncline{a9}{b9}
 \ncline{a10}{b10}
 \ncline{a11}{b11}

 \endpspicture

\end{tabular}
\caption{(Left): A connector between clause and variable gadgets.
(Right): A connector between variable gadgets.}
\label{connection_points}
\end{figure}


==> constant_factor_and_additive.tex <==
% !TEX root = uncertainalpha_journal.tex
\section{Constant-Factor and Additive Approximations}\label{sec:constant_factor_and_additive_approx}

%In this section, we derive constant factor approximation algorithms for both Problem 1 and Problem 2 where the uncertainty regions are %disks.
%
%Our approximations are based on computing minimum bottleneck spanning trees, MBSTs, which are spanning trees that minimize the maximum length edge in the tree. 
% These can be computed in $O(n \alpha(n))$ by the methods of \cite{del-edels-95}.

%Note from Erin: I removed the detailed description because I was worried about space - it can be readded for a journal version later.

%\begin{lemma} \label{lemma:bspt} A solution to the MBST problem can be found in time $O(n\log{n})$.
%%Given a set of $n$ points in the plane an MST (Minimum Spanning Tree) is also a MBST.
%\end{lemma}
%\begin{proof}
%Given an instance $I$ of MBST, consider the running of Kruskal's algorithm on $I$ for obtaining an MST.  One sorts the edges in increasing order and adds the sorted edges one at a time to get a spanning tree, not using edges which lead to cycles and stopping when a spanning tree is obtained.  We claim that any MST obtained by Kruskal's algorithm is also a MBST.
%Suppose, to the contrary, that we have a MBST, $T$, with maximum edge length $m$ and an MST, $T'$, with maximum edge length $M$, and $M > m$.  Let $e = (p,q)$ be an edge of $T'$ of length $M$.  Then, in $T$ there is a path between $p$ and $q$ consisting of edges of length less than or equal to $m$.  Let $e_1,...,e_k = (p,p_1),(p_1,p_2),...,(p_{k-1},q)$ be such a path.
%By virtue of how Kruskal's algorithm works,
%all the edges in this path either belong to $T'$, or if added to $T'$ would have created a cycle prior to the insertion of $e$.  It follows by induction that $p$ was connected to each $p_j$ and to $q$ in $T'$ even without the edge $e$, a contradiction.  Hence any MST coming from Kruskal's algorithm is also a MBST.  Kruskal's algorithm is known to run in $O(E\log{E})$ time, where $E$ denotes the number of edges in the initial graph, of which the MST is a subgraph.  Here, naively we can start with the complete graph on our $n$ points to obtain a running time of $O(n^2\log{n})$.  However, it is better to first compute the Delaunay Triangulation of the $n$ points in time $O(n\log{n})$ and utilize the fact that an MST is necessarily a subgraph of the Delaunay Triangulation.  Since the Delaunay Triangulation is a planar graph it contains at most $O(n)$ edges, and hence the total running time, starting with the Delaunay Triangulation, rather than the complete graph on the $n$ points, is $O(n\log{n})$. Since computing the Delaunay Triangulation also took time $O(n\log{n})$, the lemma is established.
%\end{proof}

%\medskip
%
%\noindent \textbf{NOTE}: This argument actually only shows that any MST obtained by Kruskal's algorithm is also a MBST.  Perhaps a perturbation argument can be used to show the more general result. (Worry about this later since it is sufficient to use the weaker result - just need to be able to find the MBST in polynomial time.)
%
%\medskip

%Our fundamental problems are the following:

%\begin{problem} (\textbf{Best Case Alpha Complex for Unit Disks}): Suppose we are given $n$ unit disks $\{D_i = D(p_i;1)\}_{i=1}^n$ in the plane with respective centers $\{p_i\}$.  Find the smallest $\alpha > 0$ such that for \textbf{some set} of locations $\ell_i \in D_i$, the union of disks $\{D(\ell_i;\alpha)\}$ is connected.
%\end{problem}

%\begin{problem} (\textbf{Worst Case Alpha Complex for Unit Disks}): Suppose we are given $n$ unit disks $\{D_i = D(p_i;1)\}_{i=1}^n$ in the plane with respective centers $\{p_i\}$.  Find the smallest $\alpha > 0$ such that for \textbf{any choice} of locations $\ell_i \in D_i$, the union of disks $\{D(\ell_i;\alpha)\}$ is connected.
%\end{problem}

We begin by considering the Best-Case  Connectivity with Uncertainty problem (BCU).

\begin{lemma} \label{lemma:best_case_opt+1} Given a set of uncertainty regions that are unit disks $D_1, \ldots, D_n$ with centers $p_1, \ldots, p_n$, let $L$ be the largest edge of a minimum bottleneck spanning tree on $\{p_i: 1 \leq i \leq n\}$.  Then choosing locations $\ell_i = p_i$ and $\alpha = L/2$ is at worst an OPT$+ 1$ approximation to the BCU Problem.  In other words, if OPT denotes the smallest radius $\alpha$ for any choice of $\ell_i \in D_i$, then $L/2 \leq $ OPT$+ 1$.
%\textbf{OLD:} This approximation can be computed in time $O(n\alpha(n))$.
This approximation can be computed in polynomial time.
\end{lemma}
\begin{proof} Consider the best choice of the $\{\ell_i \in D_i: 1 \leq i \leq n\}$ and an associated MBST on these $\{\ell_i: 1 \leq i \leq n\}$.  The edges of this MBST are each at most $2$ shorter than the corresponding edges of a spanning tree, $S$, on the corresponding $\{p_i: 1 \leq i \leq n\}$.  Thus the maximum length of any edge in $S$ is at most $2$ greater than the maximum length edge in the MBST on $\{\ell_i: 1 \leq i \leq n\}$, and, similarly, the maximum length, $L$, of any edge of an MBST on the $\{p_i: 1 \leq i \leq n\}$ must be at most $2$ greater than the maximum length edge in the MBST on $\{\ell_i: 1 \leq i \leq n\}$.  The result follows. $\Box$
\end{proof}

%{\bf Note from Erin:} Do we need Beppe's proof here?  Looks like probably not - I left it commented above in case I'm missing anything, but Jon's version seems to cover everything.

Our approximation for the BCU Problem, which we  dub the ``broadcast-from-center'' hueristic, is not necessarily a constant-factor approximation, because if one takes $n$ unit disks with non-empty intersection, then the $\ell_i$ can all be taken to equal one of the intersection points so that OPT$= 0$ while $L/2$ can be non-zero (and as big as $1$). However, we can modify our heuristic to obtain a constant-factor approximation for {\em non-overlapping} unit disks, for a result analogous to that obtained by Yang et al.~\cite{Yang07} for the case of MST with neighborhoods.

 A problem
for our heuristic, as it stands, in the case of non-overlapping disks, occurs if
we have just two disks and these two disks are within $\epsilon$ of being
tangent to one another.  As $\epsilon \rightarrow 0$ one can choose broadcast
locations $\ell_i$ increasingly close together so broadcast-from-center becomes
arbitrarily bad.  However, we can either deal with two disks as a special case,
or take the following more principled approach: begin as in
broadcast-from-center by picking the centers of all uncertainty disks, and then
find an MBST on these centers, but at the end, ``cinch-up'' any leaf nodes by
bringing the broadcast locations for these disks as close as possible to their
parent nodes.  In the case that the MBST is actually a simple path, cinch-up
twice, first at one end, then at the other.  This process ensures that we
always obtain OPT for two disks.  For three disks, we are not guaranteed to
have OPT, but because points on three unit disks cannot come arbitrarily close to
one another, the modified broadcast-from-center heuristic is a constant-factor
approximation.  See Figure \ref{3_disks}.

\begin{figure}[h]
%\centerline{\scalebox{0.45}{\includegraphics{3_disks.eps}}}
\centerline{\scalebox{0.45}{\includegraphics{3_disks_v2.eps}}}
\caption{The BCU Problem for three (almost) tangent unit disks.  OPT, as shown on the left is given by the choice of locations $(a',b',c')$, not quite on an equilateral triangle, with MBST cost $(\sqrt{1 + (\sqrt{3} - 1)^2} - 1)/2 \approx .12$, while the ``cinch-up'' heuristic, on the right, chooses locations $(a'',b'',c'')$ with cost $0.5$.}
\label{3_disks}
\end{figure}


% We need to write "modify", to indicate it is not the simple method above.

% (See the appendix, Section \ref{subsec:worstcase} for details).
%
% -- JL: This bit doesn't quite make sense to me upon rereading....
%
%We observe that the Worst Case $\alpha$ problem is likely \emph{not} in NP.  Indeed, if we had a generic polynomial time algorithm for the associated decision problem, then using a binary search, starting either with the additive approximation of Lemma \ref{lemma:worst_case_opt+1}, or the constant factor approximation of Lemma \ref{lemma:worst_case_2*opt}, we could obtain a PTAS (in fact a FPTAS).  However, the adversary's optimization problem is certainly in NP - which we can state as follows:
%
%\begin{problem} (\textbf{Adversary's Problem for Unit Disks}): Suppose we are given $n$ unit disks $\{D_i = D(p_i;1)\}_{i=1}^n$ in the plane with respective centers $\{p_i\}$.  Find locations $\ell_i \in D_i$ so that the minimum $\alpha > 0$ such that $\bigcup \{D(\ell_i;\alpha)\}$ is connected, is as large as possible.
%\end{problem}
%
%\begin{lemma} \label{lemma:adversary_opt-1} Given an instance of the Adversary's Problem for Unit Disks with disks $\{D_i = D(p_i;1)\}_{i=1}^n$, let $L$ be the largest edge of a MBST on $\{p_i\}$.  Then choosing $\ell_i = p_i$ and $\alpha = L/2$ is at worst an OPT$-1$ approximation.
%\end{lemma}
%
%\begin{proof} Same as the proof of Lemma \ref{lemma:worst_case_opt+1}.
%\end{proof}
%\medskip
%
%Just like the additive approximation from Lemma \ref{lemma:best_case_opt+1} is not necessarily a constant factor approximation, the same %is true for the additive approximation from Lemma \ref{lemma:adversary_opt-1}, since for the case of two unit disks with centers separated %by $\epsilon$, our approximation has cost $\frac{\epsilon}{2}$ while OPT has cost $\frac{1 + \epsilon}{2}$.

%\begin{lemma} Given an instance of the Worst Case Alpha Complex Problem for Unit Disks with disks $\{D_i = D_i(p_i;1)\}_{i=1}^n$, let $L$ be the largest edge of a MBST on $\{p_i\}$.  Then OPT can be as small as $\frac{\sqrt{L^2 + 4}}{2} + \epsilon$ for arbitrarily small $\epsilon$ and therefore the approximation of Lemma \ref{lemma:worst_case_opt+2} can be as bad as $2+\epsilon$ for arbitrarily small $\epsilon$.
%\end{lemma}

%Moreover, it is not hard to see that as the number of disks $N \rightarrow \infty$ our heuristic approximation gets asymptotically close to OPT.   -- THIS IS NOT AT ALL TRUE (JL): Consider the following set of disks all along a line: a pair of tangent unit disks followed by a gap the size of two tangent unit disks, followed by another pair of tangent disks, and so on, ending with a pair of tangent unit disks.  With or without cinch-up, \alpha(HEUR) = 3/2 while OPT = 1.

\section{The WCU Problem}
\label{sec:wcu}

%\medskip

We next consider the Worst-Case  Connectivity with Uncertainty (WCU) problem:
Find the minimum value $\alpha$ such that for {\em any} choice of points $P$, the connectivity graph $G_{\alpha}$ of $P$ is connected. In what follows we assume that the number, $n$, of points and associated uncertainty regions is at least $2$, since otherwise the problem is trivial.

We show a simple approximation algorithm for WCU that is within an additive
factor of 1 and a multiplicative factor of 2 when the uncertainty regions are
unit disks. Let $D(p; \lambda)$  denote the closed disk of radius $\lambda$ about the point $p$.

\begin{theorem} \label{lemma:worst_case_opt+1} Given a set of uncertainty regions that are unit disks $D_1, \ldots, D_n$ with centers $p_1, \ldots, p_n$, let $L$ be the largest edge of an MBST on $\{p_i: 1 \leq i \leq n\}$.  Then choosing $\alpha = L/2 + 1$ always results in the connectivity graph being connected and is at worst an OPT$+ 1$ approximation to the WCU Problem.
\end{theorem}

\begin{proof} First note that the connectivity graph given by any selection of $\ell_i \in D(p_i; 1)$ and $\{D(\ell_i;L/2 + 1): 1 \leq i \leq n\}$  is connected, because if $(p_i, p_j)$ is an edge of an MBST on $\{p_k: 1 \leq k \leq n\}$ then $D(\ell_i; L/2 + 1) \cap D(\ell_j; L/2 + 1) \neq \emptyset$.
% for any choice of $\ell_i \in D(p_i; 1), \ell_j \in D(p_j; 1)$.  
We are thus left to show that choosing $\alpha = L/2 + 1$ is at worst an OPT$+ 1$ approximation.  But clearly we can choose $\ell_i = p_i$ for all $i$ and so the minimum $\alpha$ is $L/2$.  Hence OPT $\geq L/2$ and the theorem is established. $\Box$
%
%So suppose $\{\ell_i\}$ is a selection of locations with $\ell_i \in D(p_i;1)$.  If $L'$ is the length of the longest edge of a MBST, $B$, on the $\{\ell_i\}$ then the corresponding spanning tree, $S$, on the $\{p_i\}$, i.e. $S = \{(p_i,p_j):(\ell_i,\ell_j) \in B\}$ has longest edge length which is no greater than $L'+2$.  It follows that the largest edge of a MBST on the $\{p_i\}$, $L$, is at most $2$ greater than the longest edge of any MBST on $\{\ell_i\}$ for arbitrary choice of $\{\ell_i\}$, and $L+2$ is at most $4$ greater than the longest edge of any MBST on such $\{\ell_i\}$.  The theorem follows.
\end{proof}

\begin{theorem} \label{lemma:worst_case_2*opt} Given a set of uncertainty regions that are unit disks $D_1, \ldots, D_n$ with centers $p_1, \ldots, p_n$, let $L$ be the largest edge of an MBST on $\{p_i: 1 \leq i \leq n\}$.  Then choosing $\alpha = L/2 + 1$  is at worst a factor $2$ approximation to OPT for the WCU problem.
\end{theorem}

\begin{proof} Note that OPT$+1 \leq 2$OPT as long as OPT $\geq 1$ so, by Theorem~\ref{lemma:worst_case_opt+1}, it suffices to show that OPT $\geq 1$.  
%If there were just one uncertainty region then our choice obviously gives OPT, hence we may assume that $n > 1$.
%By assumption there are more than one disk centers $\{p_i: 1 \leq i \leq n\}$. 
As noted in the first paragraph of this section we are assuming that $n > 1$.
Let $p_j$ be a leftmost point amongst the $\{p_i: 1 \leq i \leq n\}$ and choose $\ell_j$ to be the leftmost point in $D(p_j;1)$ and for all other  $D(p_k;1)_{k \neq j}$ choose $\ell_k$ to be the rightmost point in $D(p_k;1)$.  Then $\ell_j$ is at least distance $2$ from each of the other $\ell_k$ and so we must choose $\alpha \geq 1$ to keep the connectivity graph connected.  It follows that OPT $\geq 1$ and the theorem is established. $\Box$
\end{proof}

Theorem~\ref{lemma:worst_case_2*opt} shows that the simple broadcast-from-center heuristic can be no worse than a $2$-approximation to the solution of the WCU Problem.  However, we have thus far only found examples showing that the approximation can be (asymptotically) as bad as a $\sqrt{2}$-approximation, as the next theorem asserts.

\begin{theorem} \label{lemma:worst_case_lower_bound} Given any $L > 2$, there is an instance of the WCU Problem with uncertainty regions that are unit disks
% $\{D_i = D_i(p_i;1)\}_{i=1}^n$ 
$D_1, \ldots, D_n$ with centers $p_1, \ldots, p_n$,
such that the longest edge of an MBST on $\{p_i\}_{i=1}^n$ is $L$ and OPT is as small as $\frac{\sqrt{L^2 + 4}}{2}$, and therefore the algorithm of Theorem~\ref{lemma:worst_case_opt+1} is at best a factor $\sqrt{2} - \epsilon$ approximation for arbitrarily small $\epsilon$.
\end{theorem}


\begin{proof}
We distribute an even number of unit disks with centers equally spaced along a very large (relative to the unit disks) circle $C$.  Let us call the distance between consecutive centers of disks centered along the large circle  $L$.  We will add more disks, but $L$ will remain the longest edge of a spanning tree of the disk centers.  Additionally, let us pick $\epsilon \ll L-2$.

The construction contains a large number of highly overlapping disks in addition to the disks whose centers lie along $C$.  See Figure \ref{flower} for a sketch.
\begin{figure}[h]
\centerline{\scalebox{0.40}{\includegraphics{flower.eps}}}
\caption{The construction begins with an even number of equally spaced unit disks with centers along a very large circle $C$.}
\label{flower}
\end{figure}
The drawing is approximate in several respects.  First of all, $C$ is much, much larger than drawn, so that if the bottom of $C$ is, say, tangent to the $x$-axis, and the center of the bottom unit disk, $D_0$, has $y$-coordinate equal to $0$, then the center-points of the first unit disks to the left and right of $D_0$ along $C$, each have $y$-coordinate less than $\epsilon/3$.  In addition to the disks along $C$, there is a sequence of disks going from $D_0$ to its diametrically opposite unit disk whose centers lie along the connecting diameter. The centers of these disks are all distance $\epsilon$, one from the next, along the diameter.  If we number the $C$-centered disks in counter-clockwise order, $D_0,...,D_{2N-1}$, then we have a similar set of disks extending from each of the disks $D_2, D_4,..., D_{2N-2}$.  The key observation is that we can add such diametrically centered disks in such a way that the center of disks extending from $D_j$ to the center of $C$ are each more than distance $L$ from any other $D_k$ for $k \neq j$ -- thus the choice of $D_1$ and $D_{2N-1}$ with $y$-coordinate less than $\epsilon/3$.  On the other hand, the odd numbered unit disks $D_1, D_3,...,D_{2N-1}$, with representative element that we shall call $D_i$, each have a set of unit disks running from $D_i$ to $D_{i+2}$ with centers each $\epsilon$ from the next, but with the disks running in almost circular patterns on the outside of $C$.  An important point in this case, is that the disks start out emanating from $D_i$ along a diametric line, and then bend around so that their centers are never within $L$ of $D_{i+1}$.

We claim that for such an arrangement of unit disks, the maximum distance between locations $\ell_r \in D_r$ in a spanning tree can be as small as (and in fact slightly smaller than) $\sqrt{L^2 + 4}$, where the set $\{D_r\}$ consists not just of the disks $D_i$ with centers along $C$, but all the other unit disks depicted in Figure \ref{flower} as well.  If $D_i, D_{i+2}$ are two consecutive disks in the cyclical ordering of $C$-centered disks with $i$ odd, let $\{D_{i_k}\}$ denote the set of disks running from $D_i$ to $D_{i+2}$ outside of $C$.  Further, if $D_j, D_{j+N}$ are diametrically opposite $C$-centered disks with $j$ even, let $\{D_{j_k}\}$ denote the set of disks running diametrically between $D_j$ and $D_{j+N}$.  To verify our claim about $\{\ell_i\}$ with maximum bottleneck spanning tree edge length slightly less than $\sqrt{L^2 + 4}$, pick $\ell_i \in D_i$ for even $i$ to be the point in $D_i$ closest to the center of $C$ and $\ell_i \in D_i$ for odd $i$ to be the point in $D_i$ furthest from the center of $C$.  See Figure \ref{ells}.
\begin{figure}[h]
\centerline{\scalebox{0.50}{\includegraphics{ells.eps}}}
\caption{The distance between $\ell_i$ and $\ell_{i+1}$ (in the cyclical ordering) is just slightly less than $\sqrt{L^2 + 4}$ since the distance between successive disk centers (which we suppose to be x-axis aligned) is $L$, and the distance between the top and bottom of the successive disks, in the y-direction, is approximately $2$.}
\label{ells}
\end{figure}
Regardless of the choice of the $\ell_{i_j} \in D_{i_j}$ it is clear that $\bigcup \{D(\ell_i;\alpha)\}~\cup~\bigcup \{D(\ell_{i_j};\alpha)\}$ is connected if $2\alpha$ is the distance between consecutive locations $\ell_i, \ell_{i+1}$ (in the cyclical ordering), and that this distance is, as claimed, just slightly less than $\sqrt{L^2 + 4}$.  Let us designate this distinguished choice of the $\ell_i \in D_i$ by $\ell_i^*$, and the associated $\alpha$ by $\alpha^*$.

For these $\{D_i\}$ and $\{D_{i_j}\}$, if there were any choice of $\{\ell_i\}, \{\ell_{i_j}\}$ making $\alpha$ any larger, then we would have to pick one of the $\ell_i$ to the left or right of the diametric line through the center of $C$ and $D_i$.
It is easy to check that the result of such a choice is that there would be some cyclically ordered pair $\ell_j, \ell_{j+1}$ whose distance $d(\ell_j, \ell_{j+1}) < d(\ell_j^*, \ell_{j+1}^*) = \alpha^*$.
But then $D(\ell_j;\alpha^*) \cup D(\ell_{j+1};\alpha^*)$ connects $\ell_j, \ell_{j+1}$ and $\bigcup \{D(\ell_{2k};\alpha^*)\}~\cup~\bigcup \{D(\ell_{(2k)_j};\alpha^*)\}$ connects the even-indexed $\ell_{2k}$ and any associated choices for $\ell_{(2k)_j}$, while $\bigcup \{D(\ell_{2k+1};\alpha^*)\}~\cup~\bigcup \{D(\ell_{(2k+1)_j};\alpha^*)\}$ connects the odd-indexed $\ell_{2k+1}$ and any associated choices for $\ell_{(2k+1)_j}$.  It follows that $\alpha \leq \alpha^*$, contrary to assumption, and so the fact that OPT can be as small as $\frac{\sqrt{L^2 + 4}}{2}$ is established.
The algorithm of Theorem~\ref{lemma:worst_case_opt+1} picked $\alpha = \frac{L}{2} + 1$, so picking $L$ sufficiently close to $2$ yields $\frac{\frac{L}{2} +1}{\frac{\sqrt{L^2 + 4}}{2}} = \frac{L+2}{\sqrt{L^2 + 4}}$ sufficiently close to
$\sqrt{2}$, completing the proof. $\Box$\\%\qed
\end{proof}


%%\begin{proof}
%%  %It is easy to see that
%%  By definition, $S_1(L)$ is a subset of
%%  $U_1(L)$.
%%  %
%%  We prove by induction that $S_i(L)$ is a subset of $U_i(L)$
%%  for all $i$.
%%  %
%%  We remark that it is sufficient to prove that any open set containing a
%%  point of $S_i(L)$ intersects with the boundary of $U_i(L)$.
%% %
%%  By contradiction, let us assume that a point $p$ of $S_i(L)$ belongs to
%%  an open set $U\subseteq U_i(L)$.
%%  %
%%  We can then choose two points $q, q'  \in U$ such that $p$ is the midpoint of
%%  segment $qq'$.
%%  %
%%  Since $q\in U_i(L)$, there is a set of points
%%  $q_1,\ldots,q_i$ in $E_1,\ldots,E_i$ such that the $q_1,\ldots,q_i,q$
%%  are connected by edges of length at most $L$,
%%  %
%%  with some of them shorter.
%%  %
%%  We define $q'_1,\ldots,q'_i$ for $q'$ analogously.
%%  %
%%  For each pair $q_i$, $q'_i$, we define a continuous linear transformation
%%  $q_i(\lambda)=(1-\lambda) q_i + \lambda q'_i$, with $0\leq
%%  \lambda\leq 1$. We also define $q(\lambda)=(1-\lambda) q + \lambda
%%  q'$, so that $q(0.5)=p$. Let $l_i^2(\lambda)$ represent the square
%%  of the length of the edge connecting $q_i(\lambda)$ and
%%  $q'_i(\lambda)$. We prove that $l_i^2(\lambda)$ is a convex
%%  function. If the coordinates of $q_i$ and $q'_i$ are $(q_x,q_y)$ and
%%  $(q'_x,q'_y)$ respectively, then $l_i^2(\lambda) = (q_x+\lambda
%%  (q'_x-q_x))^2+(q_y+\lambda (q'_y-q_y))^2$. Then the second
%%  derivative is $2(q'_x-q_x)^2+2(q'_y-q_y)^2\geq 0$, and so
%%  $l_i^2(\lambda)$ is convex. So if $l_i^2(0)\leq L^2$ and
%%  $l_i^2(1)\leq L^2$, then $l_i^2(\lambda)\leq L^2$, and if one of the
%%  former inequalities is strict, then the latter also is.  Therefore,
%%  $q_1(0.5),\ldots,q_i(0.5),q(0.5)=p$ defines a list of edges of
%%  length no more than $L$, and since some of the edges connecting
%%  $q_1,\ldots,q_i,q$ are shorter than $L$, some of the edges in the
%%  path leading to $p$ are shorter than $L$. This contradicts the
%%  assumption that there is a critical path leading to $p$ with edges
%%  all of length $L$, which implies that there is no other path
%%  with shorter edges. $\Box$
%%\end{proof}
%
%%\subsection{Proof of Lemma 6}\label{subsec:l6}
%%\begin{proof}
%%  (a) This follows from the definition of $S_1(L)$. (b) By definition, $S_i(L)$ contains only points at distance $L$ from
%%  $S_{i-1}\cap E_i$. From Lemma~\ref{lem:boundary}, we know that
%%  $S_i(L)\subseteq U_i(L)$. It is therefore sufficient to prove
%%  that every point in the intersection is  in $S_i(L)$.
%%  %The case for $i=1$ is trivial, and
%%  We prove this by induction. Let $p$ be
%%  any point in the intersection. Since $p$ is in the Minkowski sum of a
%%  circle of radius $L$ and $S_{i-1}\cap E_i$, there exists $q\in S_{i-1}\cap E_i$ at distance exactly $L$ from $p$, and
%%  by the induction hypothesis, there is a path of edges of length $L$ from $q$, which
%%  we can extend to $p$. We need to prove that there is no other path
%%  to $p$ that uses edges no longer than $L$, and some shorter.
%%  %
%%  Suppose there is a choice of $p_1,\ldots,p_i$ such that $p_1,\ldots,p_i,p$
%%  is such a path. Suppose first that the last edge is shorter than $L$
%%  by some $\varepsilon>0$. Then, by changing the length of the last
%%  edge by less than $\varepsilon$, we can find paths to any point in
%%  some open set around $p$. This contradicts the assumption that $p$
%%  is part of the boundary of $U_i(L)$. Therefore, the last edge of the path is of
%%  length $L$ exactly. But that means that $p$ is at distance $L$ from
%%  both $q$ and $p_i$, which are both in $U_i(L)\cap E_i$. This means
%%  that the midpoint of the segment from $q$ to $p_i$ is in $U_i(L)\cap
%%  E_i$ and  at distance less than $L$ from $p$, yielding a contradiction. $\Box$
%%\end{proof}
%
%
%%\begin{figure}[h]
%%\begin{center}
%% \psset{unit=1cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
%% \pspicture(-1.8,-0.7)(4,4)
%%
%%% \psline[linestyle=none,fillstyle=solid,fillcolor=lightgray](2,0.5)(0.2,-0.7)(-1.8,2.3)(0,3.5)
%% \psline[linecolor=gray](2,0.5)(0,3.5)
%% \psline[linewidth=1.5pt](1,2)(4,4)
%% \uput[-30](2.5,3){segment}
%% \psline[linecolor=blue](0,0)(1,2)
%% \psline(2,1.5)(1,2)
%% \psline(1.2,3)(1,2)
%% \psdot[linewidth=1.5pt,linecolor=red](1.3,2.2)
%% \psline[linecolor=red,linestyle=dashed](0,0)(1.3,2.2)
%% \psdot[linewidth=1.5pt,linecolor=blue](1,2)
%% \psdots(0,0)(2,1.5)(1.2,3)
%%\endpspicture
%% \psset{unit=1cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
%% \pspicture(-1.8,-0.7)(4,4)
%%
%%
%% \psline[linecolor=gray](2,0.5)(-0.5,4.25)
%% \psline[linewidth=1.5pt](-0.5,1)(2.5,3)
%% \uput[-30](2.5,3){segment}
%% \psline(0.5,1)(1,2)(2,1.5)
%% \psline[linecolor=blue](0,3.5)(1,2)
%% \psdot[linewidth=1.5pt,linecolor=red](1.3,2.2)
%% \psdot[linewidth=1.5pt,linecolor=red](0.7,1.8)
%% \psline[linecolor=red,linestyle=dashed](0,3.5)(1.3,2.2)
%% \psline[linecolor=red,linestyle=dashed](0,3.5)(0.7,1.8)
%% \psdot[linewidth=1.5pt,linecolor=blue](1,2)
%% \psdots(2,1.5)(0.5,1)(0,3.5)
%%\endpspicture
%% \psset{unit=1cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
%% \pspicture(-1.8,-0.7)(4,4)
%% \endpspicture
%%
%%
%%  \pspicture(-1.8,-0.7)(4,4)
%%
%% \psline[linecolor=gray](2,0.5)(0,3.5)
%% \psline[linewidth=1.5pt](-0.5,1)(2.5,3)
%% \uput[-30](2.5,3){segment}
%% \psline[linecolor=blue](0,0)(1,2)(3,1)
%% \psline(1.2,3)(1,2)
%% \psdot[linewidth=1.5pt,linecolor=red](1.3,2.2)
%% \psdot[linewidth=1.5pt,linecolor=red](0.7,1.8)
%% \psline[linecolor=red,linestyle=dashed](0,0)(1.3,2.2)
%% \psline[linecolor=red,linestyle=dashed](3,1)(0.7,1.8)
%% \psdot[linewidth=1.5pt,linecolor=blue](1,2)
%% \psdots(3,1)(0,0)(1.2,3)
%%\endpspicture
%
%%\begin{figure}[h]%
%%%
%%\centerline{%
%%\scalebox{0.2}{\includegraphics{images/figureAlgorithmAa.eps}}%
%%\scalebox{0.2}{\includegraphics{images/figureAlgorithmAb.eps}}%
%%\scalebox{0.2}{\includegraphics{images/figureAlgorithmAc.eps}}%
%%}%
%%\caption{Points (in blue) of type $1$, $2$, and $3$ respectively, with longest incident edges in blue. In each case, moving the point along the segment results in a longer longest incident edge.}%
%%\label{fig:type}%
%%\end{figure}%
%
%
%%%%%%figures from here on in figure file%%%%%%%%%%%%%%%
%
%%\begin{figure}[h]
%%\begin{center}
%% \psset{unit=0.9cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
%% \pspicture(-2,-2)(3,2)
%% \pscircle[fillstyle=solid,fillcolor=lightgray](0,0){2}
%% \psdot[linewidth=1.5pt](0,0)
%% \uput[30](0,0){$E_1$}
%% \uput[-30](0.4,-0.5){$U_1(L)$}
%% \uput[30](1.41,1.41){$S_1(L)$}
%%\endpspicture
%%%
%% \pspicture(-3,-1.5)(3,2.5)
%% \psarc[fillstyle=solid,fillcolor=lightgray](0,0){1.4142}{135}{315}
%% \psarc[fillstyle=solid,fillcolor=lightgray](1,1){1.4142}{-45}{135}
%% \psline[linestyle=none,fillstyle=solid,fillcolor=lightgray](1,-1)(2,0)(0,2)(-1,1)
%% \psline(1,-1)(2,0)
%% \psline(0,2)(-1,1)
%% \psline[linewidth=1.5pt](0,0)(1,1)
%% \uput[-30](1,1){$E_1$}
%% \uput[-90](-0.3,-0.4){$U_1(L)$}
%% \uput[30](1.95,1.95){$S_1(L)$}
%%\endpspicture
%%\caption{Examples of $U_1(L)$ and $S_1(L)$ for the cases that $E_1$ is a fixed point
%%or a segment respectively.}
%%\label{fig:e1}
%%\end{center}
%%\end{figure}
%
%%\begin{figure}[h]
%%\begin{center}
%% \psset{unit=1cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
%% \pspicture(-1.8,-0.7)(4,4)
%%
%% \psline[linewidth=1.5pt](0,0)(3,2)
%% \psline[linewidth=1.5pt](-1,1.5)(2,3.5)
%% \psline[linecolor=red](0.5,-0.5)(1.5,1)(0.5,2.5)(-1,3.5)
%% \psline[linestyle=dashed,linecolor=blue](0.5,-0.5)(0.923077,0.61538)(-0.0769,2.1154)(-1,3.5)
%% \psdots[linewidth=1.5pt,linecolor=red](1.5,1)(0.5,2.5)
%% \psdots[linewidth=1.5pt](0.923077,0.61538)(-0.0769,2.1154)
%% \psdots(0.5,-0.5)(-1,3.5)
%% \uput[-30](0.5,-0.5){$E_1$}
%% \uput[-30](3,2){$E_2$}
%% \uput[-30](2,3.5){$E_3$}
%% \uput[30](-1,3.5){$E_4$}
%%\endpspicture
%%\caption{Choosing points (in red) on $E_2$ and $E_3$ results in a path
%%  of same-length edges. As they are of type $2$, neither can be
%%  moved without lengthening the bridging edge; yet they can
%%  be both moved simultaneously in a way that shortens some edges of
%%  the path without lengthening any other.}
%%\label{fig:par}
%%
%%\end{center}
%%\end{figure}
%
%
%
%
%%\begin{figure}[h]
%%\begin{minipage}[t]{6.75cm}
%%\begin{center}
%%\scalebox{0.11}{\includegraphics{images/figureAlgorithmBa.eps}}
%%\scalebox{0.11}{\includegraphics{images/figureAlgorithmBb.eps}}
%%\end{center}
%%%\caption[Short caption for figure 1]{\label{labelFig1} Long caption figure 1}
%%\caption{Examples of $U_1(L)$ and $S_1(L)$ for the cases that $E_1$ is a fixed point
%%or a segment respectively.}
%%\label{fig:e1}
%%\end{minipage}
%%%\hfill
%%\hspace{0.3cm}
%%\begin{minipage}[t]{7cm}
%%\begin{center}
%%\scalebox{0.11}{\includegraphics{images/figureAlgorithmC.eps}}
%%\end{center}
%%%\caption[Short caption for figure 2]{\label{labelFig2} Long caption figure 2.}
%%\caption{Choosing points (in red) on $E_2$ and $E_3$ results in a path
%%  of same-length edges. As they are of type $2$, neither can be
%%  moved without lengthening the bridging edge; yet they can
%%  be both moved simultaneously in a way that shortens some edges of
%%  the path without lengthening any other.}
%%\label{fig:par}
%%\end{minipage}
%%\end{figure}
%
%
%%\begin{figure}[h]
%%%
%%\centerline{
%%\scalebox{0.1}{\includegraphics{images/figureAlgorithmDa.eps}}
%%\scalebox{0.1}{\includegraphics{images/figureAlgorithmDb.eps}}
%%\scalebox{0.1}{\includegraphics{images/figureAlgorithmDc.eps}}
%%\scalebox{0.1}{\includegraphics{images/figureAlgorithmDd.eps}}
%%\scalebox{0.1}{\includegraphics{images/figureAlgorithmDe.eps}}
%%}
%%%
%%\caption{Shapes of $S_i(L)$ of type a, b, c, d and e respectively. $S_1(L)$ is indicated with a dashed line, $S_1(L) \cap E_2$ and $S_2(L)$ are in red.}
%%\label{fig:stype}
%%\end{figure}
%
%
%
%%\begin{figure}[h]
%%\begin{center}
%%\small
%% \psset{unit=0.8cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=3.5pt}
%% \pspicture(-0.9,1)(3.45,4.45)
%% \psline[linecolor=gray](1.5,1.25)(-0.5,4.25)
%% \uput[-150](-0.5,4.25){$P$}
%% \psline[linewidth=1.5pt](-0.5,1)(2.5,3)
%% \uput[-30](1.75,2.5){$E_2$}
%% \psline[linewidth=1.5pt](0.5,2.75)(2,3.75)
%% \uput[-30](1.25,3.25){$E_3$}
%% \psline[linewidth=1.5pt](-0.75,3)(0.75,4)
%% \uput[-30](0.75,4){$E_4$}
%% \psline[linewidth=1pt,linecolor=blue](0.5,1.25)(1,2)(0.5,2.75)(0,3.5)
%% \psdots[linewidth=1.5pt,linecolor=blue](1,2)(0.5,2.75)(0,3.5)
%% \psdots(0.5,1.25)
%% \uput[-30](0.5,1.25){$E_1$}
%%\endpspicture
%%%
%% \pspicture(-0.9,1)(3.45,4.45)
%% \psline[linecolor=gray](1.5,1.25)(-0.5,4.25)
%% \uput[-150](-0.5,4.25){$P$}
%% \psline[linewidth=1.5pt](-0.5,1)(2.5,3)
%% \uput[-30](1.75,2.5){$E_2$}
%% \psline[linewidth=1.5pt](-0.25,2.25)(1.25,3.25)
%% \uput[-30](1.25,3.25){$E_3$}
%% \psline[linewidth=1.5pt](-0.75,3)(0.75,4)
%% \uput[-30](0.75,4){$E_4$}
%% \psline[linewidth=1pt,linecolor=blue](0.5,1.25)(1,2)(0.5,2.75)(0,3.5)(0.5,4.25)
%% \psdots[linewidth=1.5pt,linecolor=blue](1,2)(0.5,2.75)(0,3.5)
%% \psdots(0.5,1.25)(0.5,4.25)
%% \uput[-30](0.5,1.25){$E_1$}
%% \uput[150](0.5,4.25){$E_5$}
%%\endpspicture
%%%
%%\pspicture(-0.9,1)(3.45,4.45)
%% \psline[linecolor=gray](1.75,0.875)(-0.5,4.25)
%% \uput[-150](-0.5,4.25){$P$}
%% \psline[linewidth=1.5pt](-0.5,1)(2.5,3)
%% \uput[-30](1.75,2.5){$E_2$}
%% \psline[linewidth=1.5pt](-0.25,2.25)(1.25,3.25)
%% \uput[-30](1.25,3.25){$E_3$}
%% \psline[linewidth=1.5pt](-0.75,3)(0.75,4)
%% \uput[-30](0.75,4){$E_4$}
%% \psline[linewidth=1pt,linecolor=blue](1.5,1.25)(1,2)(0.5,2.75)(0,3.5)
%% \psdots[linewidth=1.5pt,linecolor=blue](1,2)(0.5,2.75)(0,3.5)
%% \psdots(1.5,1.25)
%% \uput[30](1.5,1.25){$E_1$}
%%\endpspicture
%%
%%\vspace*{1cm}
%%
%% \pspicture(-0.9,1)(3.45,4.45)
%% \psline[linecolor=gray](1.75,0.875)(-0.5,4.25)
%% \uput[-150](-0.5,4.25){$P$}
%% \psline[linewidth=1.5pt](1.5,1.25)(2.25,1.75)
%% \uput[-30](2.25,1.75){$E_1$}
%% \psline[linewidth=1.5pt](-0.5,1)(2.5,3)
%% \uput[-30](1.75,2.5){$E_2$}
%% \psline[linewidth=1.5pt](-0.25,2.25)(0.5,2.75)
%% \uput[-30](-0.25,2.25){$E_3$}
%% \psline[linewidth=1.5pt](-0.75,3)(0.75,4)
%% \uput[-30](0.75,4){$E_4$}
%% \psline[linewidth=1pt,linecolor=blue](1.5,1.25)(1,2)(0.5,2.75)(0,3.5)
%% \psdots[linewidth=1.5pt,linecolor=blue](1,2)(0.5,2.75)(0,3.5)(1.5,1.25)
%%\endpspicture
%%%
%% \pspicture(-0.9,1)(3.45,4.45)
%% \psline[linecolor=gray,linestyle=dashed](1.75,0.875)(-0.5,4.25)
%% \psline[linecolor=gray,linestyle=dashed](2.125,1.125)(-0.125,4.5)
%% \uput[70](-0.5,4.25){$P$}
%% \psline[linewidth=1.5pt](1.5,1.25)(2.25,1.75)
%% \uput[-30](2.25,1.75){$E_1$}
%% \psline[linewidth=1.5pt](-0.5,1)(2.5,3)
%% \uput[-30](1.75,2.5){$E_2$}
%% \psline[linewidth=1.5pt](-0.25,2.25)(0.875,3)
%% \uput[-30](-0.25,2.25){$E_3$}
%% \psline[linewidth=1.5pt](-0.75,3)(0.75,4)
%% \uput[-30](0.75,4){$E_4$}
%% \psline[linewidth=1pt,linecolor=blue,linestyle=dashed](1.5,1.25)(1,2)(0.5,2.75)(0,3.5)
%% \psline[linewidth=1pt,linecolor=blue,linestyle=dashed](1.875,1.5)(1.375,2.25)(0.875,3)(0.375,3.75)
%% \psdots[linewidth=1.5pt,linecolor=blue](1,2)(0.5,2.75)(0,3.5)(1.5,1.25)
%% \psdots[linewidth=1.5pt,linecolor=blue](1.875,1.5)(1.375,2.25)(0.875,3)(0.375,3.75)
%%\endpspicture
%%%
%%\caption{Sequences of type I, II, III, IV and V respectively.
%%  The critical paths are shown in blue. Note that in the case of type V, the
%%  critical path can be moved at will in the indicated range. For all
%%  other sequences, any different choice of blue points on the segments
%%  results in at least one longer edge.  }
%%\label{fig:partype}
%%\end{center}
%%\end{figure}
%
%%\begin{figure}[h]
%%%
%%\centerline{
%%\scalebox{0.13}{\includegraphics{images/figureAlgorithmFa.eps}}
%%\scalebox{0.13}{\includegraphics{images/figureAlgorithmFb.eps}}
%%\scalebox{0.13}{\includegraphics{images/figureAlgorithmFc.eps}}
%%\scalebox{0.13}{\includegraphics{images/figureAlgorithmFd.eps}}
%%\scalebox{0.13}{\includegraphics{images/figureAlgorithmFe.eps}}
%%}
%%%
%%\caption{Sequences of type I, II, III, IV and V respectively.
%%  The critical paths are shown in blue. Note that in the case of type V, the
%%  critical path can be moved at will in the indicated range. For all
%%  other sequences, any different choice of blue points on the segments
%%  results in at least one longer edge.  }
%%\label{fig:partype}
%%\end{figure}
%
%%\begin{figure}[h]
%%\begin{center}
%%\small
%% \psset{unit=0.9cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=3.5pt}
%%\pspicture(-1.5,-1)(2,1.7)
%% \pscircle[fillstyle=solid,fillcolor=lightgray,linecolor=red](0.7071,0.7071){1}
%% \psarc[linestyle=dashed](0,0){1}{0}{90}
%% \psdot[linewidth=1.5pt](0,0)
%% \psline[linewidth=1.5pt](1.7142,-0.3)(-0.3,1.7142)
%% \psline[linewidth=1.5pt](1,1)(2,1)
%% \psdot[linewidth=1.5pt,linecolor=red](0.7071,0.7071)
%% \uput[210](0,0){$E_1$}
%% \uput[-90](1.7,-0.3){$E_2$}
%% \uput[-90](2,1){$E_3$}
%%\endpspicture
%%%
%%\pspicture(-1.5,-1)(2,1.7)
%% \pscircle[fillstyle=solid,fillcolor=lightgray,linecolor=red](0.7071,0.7071){1}
%% \psarc[linestyle=dashed](0,0){1}{0}{90}
%% \psdot[linewidth=1.5pt](0,0)
%% \psline[linewidth=1.5pt](1.7142,-0.3)(-0.3,1.7142)
%% \psline[linewidth=1.5pt](0.3,1.7071)(1.2,1.7071)
%% \psdots[linewidth=1.5pt,linecolor=red](0.7071,0.7071)(0.7071,1.7071)
%% \uput[210](0,0){$E_1$}
%% \uput[-90](1.7,-0.3){$E_2$}
%% \uput[90](1.2,1.7071){$E_3$}
%%\endpspicture
%%%
%%\pspicture(-1.7,-1)(2,2.8)
%% \psarc[fillstyle=solid,fillcolor=lightgray,linestyle=none](-0.3,1.8){1}{45}{225}
%% \psarc[fillstyle=solid,fillcolor=lightgray,linecolor=red](0.55,0.95){1}{-135}{45}
%% \psline[fillstyle=solid,fillcolor=lightgray,linestyle=none](0.4071,2.5071)(1.2571,1.6571)(-.1571,0.2429)(-1.0071,1.0929)
%% \psarc[linestyle=dashed](-0.45,0.95){1}{-30}{120}
%% \psdots[linewidth=1.5pt](-0.45,0.95)(0.7071,2.2071)
%% \psline[linewidth=1.5pt](1.8,-0.3)(-0.3,1.8)
%% \psdot[linewidth=1.5pt,linecolor=red](0.55,0.95)
%% \uput[210](-0.45,0.95){$E_1$}
%% \uput[-90](1.7,-0.3){$E_2$}
%% \uput[20](0.7071,2.2071){$E_3$}
%%\endpspicture
%%
%%\vspace*{1cm}
%%\pspicture(-1.7,-1)(2,1.7)
%% \psarc[fillstyle=solid,fillcolor=lightgray,linecolor=red](0.25,1.25){1}{45}{225}
%% \psarc[fillstyle=solid,fillcolor=lightgray,linecolor=red](1.25,0.25){1}{-135}{45}
%% \psline[fillstyle=solid,fillcolor=lightgray,linestyle=none](0.9571,1.9571)(1.9571,0.9571)(0.5429,-0.4571)(-0.4571,0.5429)
%% \psline[fillstyle=solid,fillcolor=lightgray,linecolor=red](0.9571,1.9571)(1.9571,0.9571)
%% \psarc[linestyle=dashed](-0.4929,0.5429){1}{45}{120}
%% \psarc[linestyle=dashed](0.5429,-0.4929){1}{-30}{45}
%% \psline[linewidth=1.5pt](0.5429,-0.4929)(-0.4929,0.5429)
%% \psline[linewidth=1.5pt](1.8,-0.3)(-0.3,1.8)
%% \psline[linewidth=1.5pt](1.4571,1.4571)(2.4571,0.4571)
%% \psline[linewidth=1.5pt,linecolor=red](1.4571,1.4571)(1.9571,0.9571)
%% \psline[linewidth=1.5pt,linecolor=red](1.25,0.25)(0.25,1.25)
%% \uput[210](0.5429,-0.4929){$E_1$}
%% \uput[70](1.7,-0.3){$E_2$}
%% \uput[-60](2.4571,0.4571){$E_3$}
%%\endpspicture
%%%
%%\pspicture(-1.7,-1)(2,1.7)
%% \psarc[fillstyle=solid,fillcolor=lightgray,linecolor=red](0.25,1.25){1}{45}{225}
%% \psarc[fillstyle=solid,fillcolor=lightgray,linecolor=red](1.25,0.25){1}{-135}{45}
%% \psline[fillstyle=solid,fillcolor=lightgray,linestyle=none](0.9571,1.9571)(1.9571,0.9571)(0.5429,-0.4571)(-0.4571,0.5429)
%% \psarc[linestyle=dashed](0.25,0.25){1}{-30}{120}
%% \psdot[linewidth=1.5pt](0.25,0.25)
%% \psline[linewidth=1.5pt](1.8,-0.3)(-0.3,1.8)
%% \psline[linewidth=1.5pt](1.4571,1.4571)(2.4571,0.4571)
%% \psdots[linewidth=1.5pt,linecolor=red](1.25,0.25)(0.25,1.25)(1.9571,0.9571)
%% \uput[210](0.25,0.25){$E_1$}
%% \uput[70](1.7,-0.3){$E_2$}
%% \uput[-60](2.4571,0.4571){$E_3$}
%%\endpspicture
%%\caption{Sequence $(E_1,E_2,E_3)$ with outcomes of type $\alpha$, $\beta$, $\gamma$, $\delta$
%%  and $\epsilon$ respectively for the case that $L$ is minimum such that $U_2(L) \cap E_3\not=
%%\emptyset$.
%%$S_1(L)$ is depicted by dashed lines. $S_1(L) \cap E_2$,
%%  $S_2(L)$ and $S_2(L) \cap E_3$ are shown in red.
%%  Note that in the outcome
%%  of type 1, a smaller $L$ would result in $U_1(L) \cap E_2 = \emptyset$,
%%  and therefore  $U_2(L) = \emptyset$. }
%%\label{fig:em}
%%\end{center}
%%\end{figure}
%
%
%%\begin{figure}[h]
%%%
%%\centerline{
%%\scalebox{0.09}{\includegraphics{images/figureAlgorithmEa.eps}}
%%\scalebox{0.11}{\includegraphics{images/figureAlgorithmEb.eps}}
%%\scalebox{0.13}{\includegraphics{images/figureAlgorithmEc.eps}}
%%\scalebox{0.13}{\includegraphics{images/figureAlgorithmEd.eps}}
%%\scalebox{0.13}{\includegraphics{images/figureAlgorithmEe.eps}}
%%}
%%%
%%\caption{Sequence $(E_1,E_2,E_3)$ with outcomes of type $\alpha$, $\beta$, $\gamma$, $\delta$
%%  and $\epsilon$ respectively for the case that $L$ is minimum such that $U_2(L) \cap E_3\not=
%%\emptyset$.
%%$S_1(L)$ is depicted by dashed lines. $S_1(L) \cap E_2$,
%%  $S_2(L)$ and $S_2(L) \cap E_3$ are shown in red.
%%  Note that in the outcome
%%  of type 1, a smaller $L$ would result in $U_1(L) \cap E_2 = \emptyset$,
%%  and therefore  $U_2(L) = \emptyset$. }
%%\label{fig:em}
%%\end{figure}
%
%%\subsection{Pseudocode of Exact Algorithm.}
%
%%\noindent\texttt{Procedure} Solve(instance,$\max$)\\
%%\vspace{0cm}\hspace{0.25cm}\texttt{if} instance contains a segment \texttt{then}\\
%%\vspace{0cm}\hspace{0.5cm}(* find critical path of instance *)\\
%%\vspace{0cm}\hspace{0.75cm} $C^*=\emptyset$\\
%%\vspace{0cm}\hspace{0.75cm}\texttt{for each} $(E_1,\ldots,E_m)$ with each $E_1,E_m$ a point or segment and $E_2,\ldots, E_{m-1}$ segments \texttt{do}\\
%%\vspace{0cm}\hspace{1cm}\texttt{if} $(E_1,\ldots,E_m)$ is a critical path candidate $C$ with longest edge-length $L_C$ and $L_C < \max$ \texttt{then}\\
%%\vspace{0cm}\hspace{1.25cm}fix points on segments in $C$\\
%%\vspace{0cm}\hspace{1.25cm}Solve(modified\_instance, $L_C$)\\
%%\vspace{0cm}\hspace{0.25cm}\texttt{else} \\
%%\vspace{0cm}\hspace{0.5cm}solve problem for point set\\
%%\vspace{0cm}\hspace{0.5cm}\texttt{if} solution is better than previous one considered \texttt{then} \\
%%\vspace{0cm}\hspace{0.75cm}save new solution for instance\\
%
%%In the search for constant-factor approximations, there is a $(\sqrt{2}, 2)$ gap established in Lemmas \ref{lemma:worst_case_2*opt} and \ref{lemma:worst_case_lower_bound} for the multiplicative constant on the broadcast-from-center heuristic.
%%Is it possible to fruitfully investigate
%% This gap could be studied experimentally.


==> figureAlgorithmAa.tex <==
 \psset{unit=0.9cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
 \pspicture(0.3,-0.2)(4,3.5)

% \psline[linestyle=none,fillstyle=solid,fillcolor=lightgray](2,0.5)(0.2,-0.7)(-1.8,2.3)(0,3.5)
 \psline[linecolor=gray](2,0.5)(0,3.5)
 \psline[linewidth=1.5pt](1,2)(4,4)
 \uput[-30](2.5,3){segment}
 \psline[linecolor=\bluecolour](0,0)(1,2)
 \psline(2,1.5)(1,2)
 \psline(1.2,3)(1,2)
 \psdot[linewidth=1.5pt,linecolor=\redcolour](1.3,2.2)
 \psline[linecolor=\redcolour,linestyle=dashed](0,0)(1.3,2.2)
 \psdot[linewidth=1.5pt,linecolor=\bluecolour](1,2)
 \psdots(0,0)(2,1.5)(1.2,3)
\endpspicture


==> figureAlgorithmAb.tex <==
 \psset{unit=0.9cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
 \pspicture(-0.6,0.3)(4,4.5)

 \psline[linecolor=gray](2,0.5)(-0.5,4.25)
 \psline[linewidth=1.5pt](-0.5,1)(2.5,3)
 \uput[-30](2.5,3){segment}
 \psline(0.5,1)(1,2)(2,1.5)
 \psline[linecolor=\bluecolour](0,3.5)(1,2)
 \psdot[linewidth=1.5pt,linecolor=\redcolour](1.3,2.2)
 \psdot[linewidth=1.5pt,linecolor=\redcolour](0.7,1.8)
 \psline[linecolor=\redcolour,linestyle=dashed](0,3.5)(1.3,2.2)
 \psline[linecolor=\redcolour,linestyle=dashed](0,3.5)(0.7,1.8)
 \psdot[linewidth=1.5pt,linecolor=\bluecolour](1,2)
 \psdots(2,1.5)(0.5,1)(0,3.5)
\endpspicture


==> figureAlgorithmAc.tex <==
 \psset{unit=0.9cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
 \pspicture(-0.5,-0.2)(3.5,3.5)

 \psline[linecolor=gray](2,0.5)(0,3.5)
 \psline[linewidth=1.5pt](-0.5,1)(2.5,3)
 \uput[-30](2.5,3){segment}
 \psline[linecolor=\bluecolour](0,0)(1,2)(3,1)
 \psline(1.2,3)(1,2)
 \psdot[linewidth=1.5pt,linecolor=\redcolour](1.3,2.2)
 \psdot[linewidth=1.5pt,linecolor=\redcolour](0.7,1.8)
 \psline[linecolor=\redcolour,linestyle=dashed](0,0)(1.3,2.2)
 \psline[linecolor=\redcolour,linestyle=dashed](3,1)(0.7,1.8)
 \psdot[linewidth=1.5pt,linecolor=\bluecolour](1,2)
 \psdots(3,1)(0,0)(1.2,3)
\endpspicture


==> figureAlgorithmBa.tex <==
 \psset{unit=0.7cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=3.5pt}
 \pspicture(-2,-2)(3,2)
 \pscircle[fillstyle=solid,fillcolor=lightgray](0,0){2}
 \psdot[linewidth=1.5pt](0,0)
 \uput[30](0,0){$E_1$}
 \uput[-30](0.2,-0.5){$U_1(\lambda)$}
 \uput[30](1.41,1.41){$S_1(\lambda)$}
\endpspicture


==> figureAlgorithmBb.tex <==
 \psset{unit=0.7cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=3.5pt}
 \pspicture(-1.5,-1.5)(3,2.5)
 \psarc[fillstyle=solid,fillcolor=lightgray](0,0){1.4142}{135}{315}
 \psarc[fillstyle=solid,fillcolor=lightgray](1,1){1.4142}{-45}{135}
 \psline[linestyle=none,fillstyle=solid,fillcolor=lightgray](1,-1)(2,0)(0,2)(-1,1)
 \psline(1,-1)(2,0)
 \psline(0,2)(-1,1)
 \psline[linewidth=1.5pt](0,0)(1,1)
 \uput[-30](1,1){$E_1$}
 \uput[-90](-0.3,-0.4){$U_1(\lambda)$}
 \uput[30](1.95,1.95){$S_1(\lambda)$}
\endpspicture


==> figureAlgorithmDa.tex <==
 \psset{unit=0.8cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=3.5pt}
 \pspicture(-0.5,-1)(2,1.7)
 \psarc[linestyle=dashed](0,0){1}{0}{90}
 \psdot[linewidth=1.5pt](0,0)
 \uput[210](0,0){$E_1$}
 \psline[linewidth=1.5pt](1.7,0)(0,1.7)
 \uput[-90](1.7,0){$E_2$}
\endpspicture

==> figureAlgorithmDb.tex <==
 \psset{unit=0.8cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=3.5pt}
\pspicture(-0.5,-1)(2,1.7)
 \pscircle[fillstyle=solid,fillcolor=lightgray,linecolor=\redcolour](0.7071,0.7071){1}
 \psarc[linestyle=dashed](0,0){1}{0}{90}
 \psdot[linewidth=1.5pt](0,0)
 \psline[linewidth=1.5pt](1.7142,-0.3)(-0.3,1.7142)
 \psdot[dotstyle=o,linewidth=1.5pt,linecolor=black](0.7071,0.7071)
 \uput[210](0,0){$E_1$}
 \uput[-90](1.7,-0.3){$E_2$}
\endpspicture

==> figureAlgorithmDc.tex <==
 \psset{unit=0.8cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=3.5pt}
\pspicture(-1.3,-1)(2,2.5)
 \psarc[fillstyle=solid,fillcolor=lightgray,linestyle=none](-0.3,1.8){1}{45}{225}
 \psarc[fillstyle=solid,fillcolor=lightgray,linecolor=\redcolour](0.55,0.95){1}{-135}{45}
 \psline[fillstyle=solid,fillcolor=lightgray,linestyle=none](0.4071,2.5071)(1.2571,1.6571)(-.1571,0.2429)(-1.0071,1.0929)
 \psarc[linestyle=dashed](-0.45,0.95){1}{-30}{120}
 \psdot[linewidth=1.5pt](-0.45,0.95)
 \psline[linewidth=1.5pt](1.8,-0.3)(-0.3,1.8)
 \psdot[dotstyle=o,linewidth=1.5pt,linecolor=black](0.55,0.95)
 \uput[210](-0.45,0.95){$E_1$}
 \uput[-90](1.7,-0.3){$E_2$}
\endpspicture

==> figureAlgorithmDd.tex <==
 \psset{unit=0.8cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=3.5pt}
\pspicture(-0.75,-1)(2,1.7)
 \psarc[fillstyle=solid,fillcolor=lightgray,linecolor=\redcolour](0.25,1.25){1}{45}{225}
 \psarc[fillstyle=solid,fillcolor=lightgray,linecolor=\redcolour](1.25,0.25){1}{-135}{45}
 \psline[fillstyle=solid,fillcolor=lightgray,linestyle=none](0.9571,1.9571)(1.9571,0.9571)(0.5429,-0.4571)(-0.4571,0.5429)
 \psarc[linestyle=dashed](0.25,0.25){1}{-30}{120}
 \psdot[linewidth=1.5pt](0.25,0.25)
 \psline[linewidth=1.5pt](1.8,-0.3)(-0.3,1.8)
 \psdots[dotstyle=o,linewidth=1.5pt,linecolor=black](1.25,0.25)(0.25,1.25)
 \uput[210](0.25,0.25){$E_1$}
 \uput[70](1.7,-0.3){$E_2$}
\endpspicture

==> figureAlgorithmEa.tex <==
 \psset{unit=0.8cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=3.5pt}
\pspicture(-0,-1)(2,1.7)
 \pscircle[fillstyle=solid,fillcolor=lightgray,linecolor=\redcolour](0.7071,0.7071){1}
 \psarc[linestyle=dashed](0,0){1}{0}{90}
 \psdot[linewidth=1.5pt](0,0)
 \psline[linewidth=1.5pt](1.7142,-0.3)(-0.3,1.7142)
 \psline[linewidth=1.5pt](1,1)(2,1)
 \psdot[dotstyle=o,linewidth=1.5pt,linecolor=black](0.7071,0.7071)
 \uput[210](0,0){$E_1$}
 \uput[-90](1.7,-0.3){$E_2$}
 \uput[-90](2,1){$E_3$}
\endpspicture

==> figureAlgorithmEb.tex <==
 \psset{unit=0.8cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=3.5pt}
\pspicture(-0.5,-1)(1.7,1.7)
 \pscircle[fillstyle=solid,fillcolor=lightgray,linecolor=\redcolour](0.7071,0.7071){1}
 \psarc[linestyle=dashed](0,0){1}{0}{90}
 \psdot[linewidth=1.5pt](0,0)
 \psline[linewidth=1.5pt](1.7142,-0.3)(-0.3,1.7142)
 \psline[linewidth=1.5pt](0.3,1.7071)(1.2,1.7071)
 \psdots[dotstyle=o,linewidth=1.5pt,linecolor=black](0.7071,0.7071)(0.7071,1.7071)
 \uput[210](0,0){$E_1$}
 \uput[-90](1.7,-0.3){$E_2$}
 \uput[90](1.2,1.7071){$E_3$}
\endpspicture

==> figureAlgorithmEc.tex <==
 \psset{unit=0.8cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=3.5pt}
\pspicture(-1.3,-1)(1.7,2.8)
 \psarc[fillstyle=solid,fillcolor=lightgray,linestyle=none](-0.3,1.8){1}{45}{225}
 \psarc[fillstyle=solid,fillcolor=lightgray,linecolor=\redcolour](0.55,0.95){1}{-135}{45}
 \psline[fillstyle=solid,fillcolor=lightgray,linestyle=none](0.4071,2.5071)(1.2571,1.6571)(-.1571,0.2429)(-1.0071,1.0929)
 \psarc[linestyle=dashed](-0.45,0.95){1}{-30}{120}
 \psdots[linewidth=1.5pt](-0.45,0.95)(0.7071,2.2071)
 \psline[linewidth=1.5pt](1.8,-0.3)(-0.3,1.8)
 \psdot[dotstyle=o,linewidth=1.5pt,linecolor=black](0.55,0.95)
 \uput[210](-0.45,0.95){$E_1$}
 \uput[-90](1.7,-0.3){$E_2$}
 \uput[20](0.7071,2.2071){$E_3$}
\endpspicture

==> figureAlgorithmEd.tex <==
 \psset{unit=0.8cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=3.5pt}
\pspicture(-0.75,-1)(2,1.7)
 \psarc[fillstyle=solid,fillcolor=lightgray,linecolor=\redcolour](0.25,1.25){1}{45}{225}
 \psarc[fillstyle=solid,fillcolor=lightgray,linecolor=\redcolour](1.25,0.25){1}{-135}{45}
 \psline[fillstyle=solid,fillcolor=lightgray,linestyle=none](0.9571,1.9571)(1.9571,0.9571)(0.5429,-0.4571)(-0.4571,0.5429)
 \psarc[linestyle=dashed](0.25,0.25){1}{-30}{120}
 \psdot[linewidth=1.5pt](0.25,0.25)
 \psline[linewidth=1.5pt](1.8,-0.3)(-0.3,1.8)
 \psline[linewidth=1.5pt](1.4571,1.4571)(2.4571,0.4571)
 \psdots[linewidth=1.5pt,linecolor=\redcolour](1.25,0.25)(0.25,1.25)(1.9571,0.9571)
 \uput[210](0.25,0.25){$E_1$}
 \uput[70](1.7,-0.3){$E_2$}
 \uput[-60](2.4571,0.4571){$E_3$}
\endpspicture

==> hardness.tex <==
\section{Hardness Results for BCU} %NEW VERSION OCTOBER 2013
\label{sec:hardness}

We prove hardness results for three variants of the BCU problem. Our first main result shows NP-hardness when the uncertainty regions are point pairs (Theorem~\ref{theorem1}). Interestingly,  this result also implies a hardness of approximation result for the case of point pairs  (Theorem~\ref{theorem2}), and NP-hardness when the uncertainty regions are line segments  (Theorem~\ref{theorem3}). Our second main result shows NP-hardness when the uncertainty regions are unit squares (Theorem~\ref{theorem4}).  We assume, in all cases, that the uncertainty regions are non-overlapping.  All of our reductions are from Planar 3-SAT -- in other words 3-SAT with the added condition that the input formula can be represented as a planar graph.


\subsection{BCU when uncertainty regions are point pairs.}
\label{sec:point-pairs}

We consider the BCU problem for uncertainty regions of vertically aligned pairs of points, unit distance apart with integer coordinates.
We study the decision version of the BCU problem for $\alpha = 1$, {\em i.e.}, we want to decide if $G_{\alpha} = G_1$ is connected for some choice of points, one for each uncertainty pair.
%
\begin{theorem}\label{theorem1} It is NP-hard to find an exact solution to the BCU problem for the case in which the regions of uncertainty are point pairs
that have a vertical distance of length one.
\end{theorem}

\begin{proof}  We show this problem is NP-hard, using a reduction from the following formulation of Planar 3-SAT. Let $\Phi = (X, C)$ be an instance of 3-SAT, with variables $X= \{x_1, \ldots, x_n\}$ and clauses $C = \{c_1, \ldots, c_m\}$.  Each clause consists of exactly three literals, each a variable or its negation.  For such an instance, we define a formula graph $H(\Phi)$ as follows: $H(\Phi) = (V, E)$ with vertex set $V =X\cup C$ and edge set $E=E_1\cup E_2$, such that $E_1 =\{(x_i,x_{i+1}) | i<n\}$, and $E_2=\{(x_i,c_j) | c_j \mbox{ contains } x_i \mbox{ or } \overline{x_i}\}$. A Planar 3-SAT instance is one whose corresponding formula graph $H(\Phi)$ is planar. In the Planar 3-SAT problem, our goal is to determine whether a given Planar 3-SAT instance $\Phi$ is satisfiable. This problem is known to be NP-complete \cite{Garey_Johnson79,Lichtenstein}.

Our reduction makes use of the fact that, given a Planar 3-SAT instance $\Phi$ with formula graph $H(\Phi)$, this graph has a planar layout on an $O(n+m) \times O(n+m)$ grid~\cite{Duchet,Rosenstiehl}.  Further, in this layout, the vertices (variables and clauses) can be drawn as horizontal line segments and edges as vertical line segments.  Henceforth, we equate the formula graph $H(\Phi)$ with the planar layout we have described above.

To reduce from Planar 3-SAT to  BCU when the uncertainty regions are pairs of points, we design various gadgets.  Specifically, given a layout of a Planar 3-SAT instance using line segments as described above, we replace each horizontal line segment corresponding to a variable by a variable gadget, each horizontal line segment corresponding to a clause by a clause gadget, and each vertical line segment corresponding to an edge in $E_1$ by a variable-variable connector and each one corresponding to an edge in $E_2$ by a variable-clause connector.  Below we will argue that there exists a choice of point in each of these uncertainty pairs such that the connectivity graph for $\alpha = 1$, $G_1$, is connected if and only if the corresponding Planar 3-SAT instance is satisfiable.

%\medskip

\subsubsection*{Overview of the gadgets}
We  present the main ideas behind the clause gadgets, variable gadgets, and connector gadgets mentioned above.

A clause gadget is designed so that it contains three ``gates'', one for each of the literals in the clause. The gate for each
literal is either on the top or the bottom of the clause gadget, depending on whether the literal appears above or below the
clause in the planar grid layout of $H(\Phi)$. For the connectivity subgraph corresponding to the
clause to be connected to the rest of the graph in $G_1$, at least one of these three gates must be open. This corresponds
to setting the literal to \true\ in the clause. This, in turn, ensures that the clause is satisfied. %See Figure~\ref{clause_gadget_points}.

The role of a variable gadget is to choose and propagate a truth value
for the variable to all the clauses containing it in a consistent
manner. The variable gadget contains three types of constructs. Type
$I$ and type $II$ constructs help link the variable to all the clauses
that contain it and are either above or below it. We have one such
type $I$-type $II$ pair for every occurrence of the variable in a
clause. A construct of type $III$ is used to ensure that the subgraph
corresponding to the variable gadget can be connected if and only if
the truth assignment to the variable in all the copies of type
$I$-type $II$ pairs are the same.  Our construction also prevents
subgraphs arising from parts of a variable gadget from being connected
through other parts of
$G_1$. %See Figure~\ref{vble_gadget_points} in the Appendix (Section \ref{subsec:pointpairs}).

The variable and clause gadgets are linked to each other using two
types of connectors. A clause-variable connector replaces an edge of
$H(\Phi)$
between a clause vertex and a variable vertex in such a way that
points chosen in the corresponding gadgets can be connected through it
if and only if the truth value of the variable is consistent with its
occurrence (as a literal) in the clause.  A variable-variable
connector replaces an edge of $H(\Phi)$
between two variable vertices. Points in one variable gadget can be
connected to those in another variable gadget via points chosen in the
variable-variable connector irrespective of the choice of truth values
for each variable gadget. %See Figure~\ref{connection_points} in the Appendix (Section \ref{subsec:pointpairs}).

Having given the overview of the reduction, we now provide a detailed proof by first describing the different  gadgets in detail and then  arguing the correctness of our reduction.

\subsubsection*{The clause gadget}
%ALEJANDRO 2015-03-27:  I diffed this subsubsection with the Arxiv version and integrated relevant changes.

Figure~\ref{schema_clause_points} depicts a schema that describes the functioning of a clause gadget.  Each gate in the schema represents the entry of a connection to a literal, with an open gate representing a contribution of \true.  If all gates are closed, then, as suggested by the schema, it is possible that the connectivity graph of the clause gadget is connected, but it is isolated from the rest of the graph.  Also, as the schema suggests,  if gates to two literals $x_i$ and $x_j$ are both open, then connections are created between the clause gadget and the gadgets for the literals, but no connection via the clause gadget is made between the variable gadgets.

\input{schema}

The shape of the clause gadget can be adapted to meet the requirements of the clause vertex it represents in the planar layout of $H(\Phi)$ (e.g., the length of the horizontal line segment representing a particular clause gadget in the planar layout of $H( \Phi )$ by line segments;  however many of the horizontal segments representing literals contained in the clause lie below the segment representing the clause and however many above).  Figure~\ref{clause_gadget_points} shows an example of a clause gadget where, in the representation of $H (\Phi )$, the clause was represented by a horizontal segment connected to one horizontal variable segment lying above, and two horizontal variable segments lying below the segment for the clause. The clause gadget is flexible, as its size can be adjusted by adding more uncertainty pairs to the sequence between two connections to the variable gadgets, and to the sequence between connections to variable gadgets and the left and right sides of the gadget.  Furthermore, in a straightforward manner we can modify the clause gadget to move the connection to a particular variable gadget vertically by one unit without moving the entire clause gadget; e.g., the uncertainty pairs in the gray box in Figure~\ref{clause_gadget_points} can be moved up by one unit.

Consider the three uncertainty pairs with white and gray points in Figure~\ref{clause_gadget_points}.  If all three of the white points are chosen, then it is easy to see that, while points can be chosen so that the connectivity subgraph arising from pairs in the clause gadget can be made connected, no such subgraph can be connected to the rest of $G_1$ for any choice of points in the remaining uncertainty pairs. If a gray point is chosen from a white-gray pair, then the dashed edges shown incident to the pair do not belong to  $G_1$.

\input{clauseGadgetPoints}

Each of the three white-gray uncertainty pairs is connected to a variable gadget by a sequence of vertical uncertainty pairs.  The choice of a gray point, shown in the schema as an open gate, is intended to mean that the literal (a variable or its negation) connecting to this open gate contributes a \true\ to the clause.  Note that the clause gadget never connects two variable gadgets.

Next, we outline how variable gadgets transmit truth values and how consistency of truth assignments is assured.


\subsubsection*{The variable gadget}
% ALEJANDRO 2015-03-27: I have diffed this \subsubsection*{The
% variable gadget} with Arxiv version and integrated relevant changes.
An example of the variable gadget is shown in
Figure~\ref{vble_gadget_points}.  Let the uncertainty pair at the
extreme left of the variable gadget be the \emph{reference pair} for
this variable.  We adopt the interpretation that the choice of black
point in the reference pair means a setting of \true\ to the variable
and the choice of gray point means a setting of \false\ to the
variable.

\input{variableGadgetPoints}

In order for the constructs of type $I$, $II$, and $III$ to function
as described above, in the Overview of the gadgets, we require that
the following two properties hold: (1)
%for any choice of points in all uncertainty pairs,
%no cycle of $G_1$ contains a pair of non-consecutive vertices in variable gadgets;
for all variable gadgets, $G_1$ is connected only if the subgraph of
$G_1$ restricted to points chosen in a given variable gadget is
connected; and, (2) the subgraph of $G_1$ restricted to points chosen
in a variable gadget can be connected if and only if the truth values
in type $I$ and $II$ constructs are consistent with the reference pair
(as these are the parts of the gadget that propagate truth values to
clause gadgets).  Together, these properties ensure that for $G_1$ to
be connected, the points chosen from variable gadgets must be
internally connected and, in turn, each variable gadget must propagate
consistent truth values to the clause gadgets that are connected to it
via connector gadgets. We prove these two properties now.

% The variable gadget consists of constructs of type $I$, $II$ and $III$.
% %
% %For $G_1$ to be connected, the subgraph of $G_1$ arising from a variable gadget %must be internally connected as it is not possible to join parts of it using paths %running through subgraphs arising from clause gadgets or other variable gadgets.
% %
% Therefore, the choice of any black point in a construct of type $I$ or $II$ forces the choice of black points in this as well as in all the other constructs of type $I$ and $II$ inside this variable gadget. The same is true for gray points.  In Figure~\ref{vble_gadget_points}, if the gray point is chosen in the reference pair, gray arrows show the implications that force the choice of gray points in all the type $I$ and $II$ constructs.  The function of the type $III$ construct in the variable gadget is to allow this propagation.

Recall that the clause gadget connects to the literals that
are satisfied (only) by opening gates, and that no two open gates are
connected through the clause gadget.  As such, there cannot be a path
in $G_1$ joining points in two (possibly indistinct) variable gadgets through points in a
clause gadget.  In addition, the edges $E_1$ join the variable
vertices (horizontal lines) in $H(\Phi)$ by a path, not a cycle.
Therefore, $G_1$ can be connected only if the subgraph of $G_1$ corresponding to points chosen from any variable gadget is connected.
 %no two non-consecutive vertices of a cycle in $G_1$ are in variable gadgets.
This shows the first property.

The choice of any black point in a construct of type $I$ or $II$
forces the choice of black points in this as well as in all the other
constructs of type $I$ and $II$ inside a variable gadget.  The same is
true for gray points.  In Figure~\ref{vble_gadget_points}, if the gray
point is chosen in the reference pair, gray arrows show the
implications that force the choice of gray points in all the type $I$
and $II$ constructs.  The function of the type $III$ construct in the
variable gadget is to allow this propagation.  Thus, the second
property holds; the variable gadget can be internally connected if and
only if the truth value of the reference pair agrees with the truth
value in type $I$ and type $II$ constructs.

% The construction of the
% variable gadget ensures the required internal connectedness in such a
% way that for any choice of points $P$ from the uncertainty pairs, a
% necessary and sufficient condition for the subgraph of the
% connectivity graph $G_1$ of $P$ restricted to a variable gadget to be
% connected is that the points in $P$ represent a consistent choice of
% truth value for this variable.

% Considering that uncertainty pairs in the variable gadget cannot be connected via a path though another variable or a clause gadget, we conclude that the variable gadget is designed in such a way such that the pairs in the gadget are connected iff there is a consistent truth assignment to this variable in all the clauses.

%  This follows from the observation that a clause gadget cannot connect two different clause-variable connectors.


% ALEJANDRO 2015-03-27:  Note that I have not adopted the new Arxiv stuff here, as the old stuff is ok, and the new stuff needs editing.
% \old{For any choice of points $P$ from the uncertainty pairs, a necessary and sufficient condition for the subgraph of the connectivity graph $G_1$ of $P$ restricted to a variable gadget to be connected is that the points in $P$ represent a consistent choice of truth value for this variable. This follows from the observation that a clause gadget cannot connect two different variable gadgets.}

% ALEJANDRO 2015-03-27: The ArXiv stuff does not make sense to me, but it does highlight the need for a change re. the internal connectedness of the variable gadget.
% \new{Considering that pairs in the variable gadget cannot be connected via a path though another variable or a clause gadget, we conclude that the variable gadget is designed in such a way such that the pairs in the gadget are connected iff there is a consistent truth assignment to this variable in all the clauses.}

We describe how the type $I$ and type $II$ constructs are used to
connect to clause gadgets above and below the variable gadget.
Suppose that the variable associated with this gadget is $x$.  If the
literal $x$ appears in a clause gadget embedded above the variable
gadget, then the connection from the corresponding clause gadget to
this variable gadget (to be described in the next section) is made to
the top of a construct of type $I$. In order to connect the variable
gadget to the clause gadget, a black point has to be chosen in the
reference pair.  If the literal $\overline{x}$ appears in a clause
above the variable gadget, then the connection is made to the top of a
construct of type $II$ and a gray point is chosen in a reference
pair. Similarly, if the literal $x$ appears in a clause embedded below
the variable gadget, the connection from the clause gadget is made to
the bottom of a type $II$ construct and the black point is chosen in
the reference pair. If the literal $\overline{x}$ appears in a clause
embedded below the variable gadget, the connection is made to the
bottom of a type $I$ construct and the gray point is chosen in the
reference pair.

We replace horizontal line segments corresponding to variables in the embedding of the Planar 3-SAT instance by variable gadgets. Note that the width of type $I$ and $II$ constructs can be adjusted by adding horizontally arranged uncertainty pairs.
The number of occurrences of constructs of type $I$, $II$ and $III$ depends on the number of clauses containing this variable.

\subsubsection*{Linking the gadgets}
% ALEJANDRO 2015-03-27: I have diffed \subsubsection*{Linking the gadgets} with Arxiv version and integrated relevant changes.  In particular, the discussion of moving clause gates up or down.
We now explain how to represent the edges of the planar graph
$H(\Phi)$, corresponding to an instance $\Phi$ of Planar 3-SAT.  In
the embedding we are considering, edges are represented by vertical
line segments.  They represent two kinds of connections: (1) between a
pair of variables, and (2) between a clause and a variable in that
clause.  Figure~\ref{connection_points} shows vertical constructs of
uncertainty pairs that (right) connect pairs of variable gadgets and
(left) clause and variable gadgets. We observe the following
properties of the two connectors: In a clause-variable connector, the
choice of black point in a clause gadget above a variable gadget
implies the choice of black point in the variable gadget. The choice
of gray point in the clause gadget below a variable gadget forces the
choice of gray point in the variable gadget. In the variable-variable
connector, for any choice of points in the two vertically extreme
uncertainty pairs, there is a path using points in the shown
uncertainty pairs that connects the two extreme uncertainty pairs.
The white uncertainty pair allows this connection. The $n$ variable
gadgets are connected using $n-1$ variable-variable connectors that
replace $E_1$ in $H(\Phi)$.

\input{connector}

% [OLD]
% \noindent Note that the positions of the tops of constructs I and II
% in the variable gadget differ vertically by one unit; therefore, we
% ensure that the positions of two gates on the same side of a clause
% gadget can also differ vertically by one unit, if necessary.  An
% example of this is shown in Figure~\ref{clause_gadget_points} and,
% evidently, the gates may also be positioned at the same height
% instead.

% [NEW] adapted from ArXiv
Note that the parities of the (integer) heights of the tops of type I
and type II constructs in the variable gadget differ (see
Figure~\ref{vble_gadget_points}); we must ensure that clause gadgets
have the flexibility to accommodate this.  Indeed, this is the case;
consider again Figure~\ref{clause_gadget_points}.  If necessary,
gate-constructs can be shifted vertically by one unit to allow such
connections.  For example, the gate on the top of the gadget in
Figure~\ref{clause_gadget_points} can be shifted by moving all the
uncertainty pairs in the gray box up by one unit.  This change
preserves the properties of the clause gadget given earlier.

\subsubsection*{Correctness of the reduction}
In a line segment embedding of the planar graph $H(\Phi)$
corresponding to a Planar 3-SAT instance $\Phi$, nodes (clauses and
variables) are horizontal line segments and edges are vertical line
segments.  We have presented clause and variable gadgets to replace
horizontal line segments and connectors to replace vertical line
segments.  We argue that the connectivity graph $G_1$ is connected for
some choice of points in these uncertainty pairs if and only if the
Planar 3-SAT instance $\Phi$ is satisfiable.

If the Planar 3-SAT instance $\Phi$ is satisfiable, let us consider the assignment of truth values to the variables of the instance.  When a variable is set to \true, we choose the black point in the reference pair of the corresponding variable gadget.  When it is set to \false, we choose the gray point.
% removed as per ArXiv
% This leads, in turn, to the appropriate choice of points in the connectors and inside the clause gadgets.
Let $P$ be the set of points chosen and consider the graph $G_1$ of $P$. In $G_1$, points selected in variable gadgets are all internally connected and connected to each other via the variable-variable connectors.  As all the clauses are satisfied by the truth assignment, each clause is connected to one or more variable gadgets through edge-disjoint paths. Therefore the graph $G_1$ is connected.

Suppose that there exists a choice of points in $U$ such that its corresponding connectivity graph $G_1$ is connected.
In $G_1$, points in each clause gadget are connected to points in one or more variable gadgets through edge-disjoint paths. Therefore, points in two different variable gadgets can never be connected via a path that includes points chosen from a clause gadget.
%ALEJANDRO: my change here subsumes the ArXiv concern about path of length n-1.
This implies that if $G_1$ is connected, then all the internally connected variable gadgets are connected to each other via the path in $H(\Phi)$ that is replaced by the $n-1$ variable-variable connectors.
%
%% Svetlana: internal connectedness argument is for points in the same variable gadget, not two different ones
%
A truth value is assigned to each variable solely depending on whether the black or gray point is chosen inside the variable gadget. Since every clause gadget is connected to at least one variable gadget, the truth assignment satisfies every clause.  Therefore, this truth assignment satisfies the Planar 3-SAT instance $\Phi$.

% ALEJANDRO: This is just the contrapositive of the above.  not
% needed.
% Conversely, if there is no satisfying assignment to the
% Planar 3-SAT instance, then $G_1$ cannot be connected.  In
% particular, part of a clause gadget corresponding to an unsatisfied
% clause (with respect to a given truth assignment) cannot be
% connected to the rest of the graph using edges of length at most
% $2$.

This proves Theorem~\ref{theorem1}. \hfill$\Box$
\end{proof}
%


%By reduction from Planar 3-SAT, BCU for non-overlapping uncertainty regions that are pairs of vertically aligned points one unit apart with integer coordinates is NP-hard.

%----------------------------------------------------------



\subsection{Inapproximability for point pairs}
\label{subsec:best}
We observe that for uncertainty regions that are pairs of points,
there is no approximation algorithm, polynomial in the size of the
input, with an approximation ratio less than $\sqrt{5}/2$, unless
$P=NP$.  Indeed, we have provided problem instances where the
uncertainty regions are vertically aligned pairs of points separated
by a distance of one unit such that a Bottleneck Spanning Tree of
maximum edge length $2$ ($\alpha = 1$) can be found if and only if
$P = NP$.  But two points on the integer grid, if further apart than
distance $2$, must be at least distance $\sqrt{5}$ from one another.
Hence if we had a polynomial time approximation to the solution with a
ratio less than $\sqrt{5}/2$ then we could use the approximation to
find a Bottleneck Spanning Tree with maximum edge length not greater
than $2$, a contradiction (unless $P = NP$).

\begin{theorem} \label{theorem2}
There  is no approximation algorithm, polynomial in the size of the input, that solves BCU for point pairs with approximation ratio  less than $\sqrt{5}/2$, unless $P=NP$.
\end{theorem}





\subsection{BCU when the uncertainty regions are line segments}
\label{subsec:line}
We can also prove that the BCU problem is NP-hard for vertical unit segments on an integer grid.  To show this,  we use the same argument as in the proof of Theorem~\ref{theorem1} except that point pairs, unit distance apart, are now replaced by vertical line segments of unit length.

\begin{theorem} \label{theorem3}
It is NP-hard to find an exact solution to the BCU problem for the case in which the regions of uncertainty are vertical unit edges.
\end{theorem}

\noindent Hardness of approximation, such as for point pairs (Theorem~\ref{theorem2}), however, does not hold for line segments, because we can use edges of length arbitrarily close to $2$.


\subsection{BCU when the uncertainty regions are unit squares}% SIXTWO

We prove an NP-hardness result for this problem using a reduction from
Planar 3-SAT. Our reduction uses techniques similar to the previous
reduction.

\begin{theorem}\label{theorem4}
It is NP-hard to find an exact solution to the BCU problem for the case where the regions of uncertainty are unit squares.% of edge length one.
\end{theorem}

\begin{proof}
  We use a reduction from the formulation and embedding $H(\Phi)$ of a Planar
  3-SAT instance $\Phi$ that is given in the proof of Theorem~\ref{theorem1}.

  We need the following terminology:
A point $p$ is \emph{$l$-connected} to a point $q$ if the (Euclidean) distance from $p$ to $q$ does not exceed $l$.  A set $S$ of points is $l$-connected if the maximum edge length of the minimum spanning tree of $S$ does not exceed $l$.

We now describe the variable and the clause gadgets as well as the connectors we use to link the variables and clauses.

\subsubsection{The variable gadget.}
For each variable, we create a gadget similar to the one shown in
Figure~\ref{fig:variablegadget}.  The variable gadget, as shown in the
figure, can be $5$-connected in two ways: by choosing the \redcolour\
points in each square, or by choosing the \bluecolour\ points in each
square.  We call the bold square in the figure the \emph{reference}
square.  A point in the reference square can only be 5-connected to a
point in at most one square among the other squares in the variable
gadget.  If the \bluecolour\ point is chosen to make this connection
in the reference square, then we say that the variable associated with
this gadget is \true; if the \redcolour\ point is chosen, we say that
the variable is \false.  Furthermore, the subgraph of $G_1$
corresponding to points in a variable gadget can be connected if and
only if the points (black or gray) chosen for all of its uncertainty
regions are consistent.

\input{variableGadgetSquares}

Connections to clause gadgets (which replace clause vertices embedded
as horizontal lines) that contain this variable or its negation are
made via constructs similar to the four extreme top and bottom squares
shown in the example variable gadget of
Figure~\ref{fig:variablegadget}.  Of these, the top left and bottom
right connect to clauses containing this variable and the top right
and bottom left connect to clauses containing the negation of this
variable.  The width of the variable gadget can easily be increased
and more such constructs can be added to allow additional connections
(which replace edges embedded as vertical lines of $H(\Phi)$) to
clause gadgets above or below.

\subsubsection{The clause gadget.}

For each clause, we create a gadget such as the one shown in
Figure~\ref{fig:clausegadget}.  We call the bold square in the clause
gadget the \emph{core} square.  For each of the 3 literals (a variable
or its negation), there is a sequence of squares in the gadget, called
an \emph{arm}.

Observe that the core square can be $5$-connected to only a single arm, and once this arm is selected, the choice of points in its squares is \emph{fixed} in order for the squares to be $5$-connected.  The choice of points within the other arms' squares is \emph{free} since they do not need to connect to the core point.  These squares can be made connected to each other.

\input{clauseGadgetSquares}

\subsubsection{Linking the gadgets.}
Here we explain how variable gadgets can be linked to clause gadgets and how variable gadgets can be linked to each other.

Clause-variable connectors represent edges of $H(\Phi)$
and, as such, they propagate truth values vertically. In order to
attach them to the horizontal arms of the clause gadget, shown in
Figure~\ref{fig:clausegadget}, we use a corner gadget, shown in
Figure~\ref{fig:linkgadget}, to change the alignment of the
\redcolour\ and \bluecolour\ points in the square regions from
horizontal to vertical.  The corner and clause gadgets may be
reflected as necessary in order to attach to three clause-variable
connectors above and/or below the clause gadget.

% We may also require horizontal and vertical
% reflections of corner gadgets. Likewise, the corner gadget enables
% connections to variable gadgets above the clause gadget.  To connect
% the lower arm of the clause gadget to a variable gadget above the
% clause gadget, two corner gadgets are necessary.

\input{linkingGadgetSquares}

To complete the connection between vertex and clause gadgets, it remains to explain how to connect pairs of square uncertainty regions, one in the variable gadget and the other in an extension of one of the arms of the clause gadgets.  We would like to propagate truth assignments (choice of \redcolour\ or \bluecolour\ point in the variable gadget) consistently along such connectors.  When the distance between the points to be joined in the two squares is a multiple of $5$ and these points are vertically aligned, the connection can be made in the way analogous to that shown in Figure~\ref{connection_points}(Left).  Otherwise the construction of such connectors can be easily accomplished but is quite tedious to describe.  We leave this construction to the reader.  %EXAMPLE HERE.

To connect variable gadgets to each other (in place of the edge subset
$E_1$ of the Planar 3-SAT embedding), we add $n-1$ \emph{loose}
connections between the $n$ variable gadgets by using a sequence of
squares that allow the variable gadgets to be $5$-connected to each
other, regardless of the choice of point in the squares of the
gadget.
%Figure~\ref{fig:forestlink} shows an example of such a connection.
Figure~\ref{fig:forestlink} shows such a loose connection between two horizontal sequences of squares.  The variable gadgets may need to be expanded by adding horizontal sequences of squares in order to allow these connections.

\input{connectingGadgetsSquares.tex}

\subsubsection{Correctness of the Reduction.}

We now argue that there exists a choice of point in each of the square uncertainty regions such that the connectivity graph for $\alpha = 5/2$ is connected if and only if the corresponding Planar 3-SAT instance is satisfiable.

Suppose that there is a satisfying assignment to the Planar 3-SAT
instance.  Then, in each variable gadget we choose the \bluecolour\
corner of the reference square when that variable is \true\ and the
\redcolour\ corner when that variable is \false\ in the satisfying
assignment.
% ALEJANDRO: tying in with things explained in Thm 1 argument
Our construction shares the property with the one in
Section~\ref{sec:point-pairs}, for point-pairs, that points chosen in a variable gadget
must be internally connected for $G_1$ to be connected.  As such, we
must choose points in the other squares of the variable gadgets to be
the same colour as that of the reference square.
%
The choice of
\redcolour\ or \bluecolour\ point is then propagated to every clause
gadget satisfied by this assignment via the connectors.  Note that the
truth value is correctly inverted by the variable gadget when
connecting a negated variable to a clause that includes this literal.
Since all the clauses are satisfied, the core square in each clause
gadget is connected to a variable that satisfies the clause.  The arms
that do not connect to the core square are connected to their
respective variable gadgets.  At this point we have created $n$ trees,
one for each variable.  Points chosen in $n-1$ connectors between variable gadgets
make $G_{5/2}$ connected.

Let $P$ be any choice of points in the square regions for which the corresponding graph $G_{5/2}$ is connected.  Since $G_{5/2}$ is connected, points in each clause gadget are connected to points in exactly one variable gadget.  Because variable gadgets can never be connected to each other via a clause gadget, each variable gadget must be internally connected.  The choice of \redcolour\ or \bluecolour\ point in the reference square of each variable gadget assigns the satisfying truth assignment to the variable associated with that variable gadget in the Planar 3-SAT instance.

% Conversely, if there is no satisfying assignment to the Planar 3-SAT
% instance, then $G_{5/2}$ cannot be connected.  In particular, the core
% square of a clause gadget corresponding to an unsatisfied clause (with
% respect to a given truth assignment) cannot be connected to the clause
% gadget's arms using edges of length at most $5$.

By reduction from Planar 3-SAT, BCU for non-overlapping unit square uncertainty regions whose corners can be given integer coordinates is NP-hard.\hfill$\Box$
\end{proof}

\noindent Once again, hardness of approximation does not hold because we can use
edges of length arbitrarily close to $5$.



==> intro.tex <==
\section{Introduction}\label{sec:intro}

Finding an optimally connected substructure in a network is one of the fundamental combinatorial optimization problems in network design. The standard problem of minimizing the total edge cost in the network amounts to finding a minimum spanning tree, which can be computed by straightforward greedy methods. A closely related problem that has gained in importance in the context of wireless networking is to consider the ``bottleneck'' problem of minimizing the length of the longest edge. 
%This corresponds to choosing the necessary power and thus range for the routers to be placed at nodes. Often, greedy methods still yield optimal solutions.
A solution to this problem allows one to choose a point set of lowest power, where equi-power routers are to be placed at nodes, such that a message can be relayed between any two nodes.
%
However, the situation changes when the locations of devices becomes part of the problem: How should each location be chosen from a given neighborhood, such that the solution to the resulting bottleneck connectivity problem is minimized? The neighborhoods can be the result of imprecise input data, or simply arise from a geometric range of possible locations; depending on the scenario, the choice of locations can be optimistic (i.e., best case) or adversarial (i.e., worst case).


Let $U$, $|U|=n$, denote a family of uncertainty regions, e.g., a family of disks, squares, line segments or pairs of points.  For each uncertainty region $u_i \in U$, $1 \leq i \leq n$, one point $p_i$ is to be chosen inside this region $u_i$.  Let $P$ be the set of points chosen. For a value $\alpha \in \mathbb{R}$, we define the {\em connectivity graph} $G_{\alpha}=(V,E)$ of $P$ with respect to $\alpha$ as follows: $V=P$ and $E = \{ (p_i, p_j)\in P\times P, \|p_i-p_j\|_2 \leq 2\alpha\}$.  Thus, the graph connects a pair of points with an edge whenever closed disks of radius $\alpha$ centered at these points intersect. We can now formally define the main problem, {\em Best-Case Connectivity with Uncertainty} (BCU), that we study in this paper.\\

\noindent
{\bf The BCU Problem.}
\label{problem2}
Given a set $U=\{u_1,\ldots, u_n\}$ of $n$ uncertainty regions, find the minimum value $\alpha$ for which there exists a choice of point set $P=\{p_1,\ldots, p_n\}, p_i \in u_i$, such that the connectivity graph $G_{\alpha}$ of $P$ is connected.
%\end{problem}

\medskip
\noindent We further study a closely related problem, {\em Worst-Case  Connectivity with Uncertainty} (WCU):\\

\noindent
{\bf The WCU Problem.}
Given a set $U=\{u_1,\ldots, u_n\}$ of $n$ uncertainty regions, find the minimum value $\alpha$,
such that for {\em any} choice of point set $P=\{p_1,\ldots, p_n\}, p_i \in u_i,$ the connectivity graph $G_{\alpha}$ of $P$ is connected.

%Problem 2 Best Case á: Given n uncertainty regions, find the minimum radius á such that there
%exists a set of points from the regions whose connectivity graph is connected.

\subsection{Related Work.}
%\textbf{OLD:} If the $n$ uncertainty regions are points (in other words, there is no uncertainty),
%%If we are given a set of $n$ points instead of $n$ uncertainty regions,
%an efficient algorithm is known for finding the minimum $\alpha$ for which the
%connectivity graph is connected. The algorithm, due to Delfinado and
%Edelsbrunner \cite{del-edels-95}, has a running time of $O(n\alpha(n))$, where
%$\alpha(n)$ denotes the inverse of the Ackermann function.
%
If the $n$ uncertainty regions are points (in other words, there is no uncertainty),
%If we are given a set of $n$ points instead of $n$ uncertainty regions,
then finding the minimum $\alpha$ for which the connectivity graph is connected amounts to finding a
minimum Euclidean Bottleneck Spanning Tree (MBST) on the points.  Because minimum spanning trees
(MSTs) are also MBSTs, a solution can be found in time $O(n\log{n})$.

Closely related to our BCU and WCU problems is the well-studied family
of {\rm range assignment} problems.  In these problems, the disks
centered at the points can be of different radius, and the goal is to
minimize the total power consumption under the constraint that the
network satisfies certain structural properties like connectivity,
strong connectivity, or a particular broadcast property.
 %The exact expression being minimized depends on the distance-power gradient.
 Most of the work on these problems has considered point sets rather than
uncertainty regions (see \cite{cps-opapr-00,lp-eaasb-02,lp-ptasb-05,SCG06,fuchs-06}).
 %For literature on this type of problems see for example \cite{cps-opapr-00},
 %\cite{lp-eaasb-02}, \cite{lp-ptasb-05}, %\cite{SCG06} and \cite{fuchs-06}.
%
Thus our work provides an early exploration of connectivity problems, arising in the context of wireless networks, for points lying in nontrivial uncertainty regions.

The minimum spanning tree problem (MST) has been studied in the setting of
uncertainty regions. Yang {\em et al.} \cite{Yang07} showed that the problem of
computing a spanning tree that minimizes the total edge length is NP-hard if
the uncertainty regions are non-overlapping unit disks or rectangles. They also
give a polynomial-time approximation scheme (PTAS) for the case in which the
uncertainty regions are unit disks; this is notably different from our problem,
which does not admit a PTAS, unless P=NP. Further approximation results
for minimization and maximization versions of the MST with uncertainty were provided by 
Dorrigiv \emph{et al.}~\cite{dfh+-mmwst-12}.
Another optimization problem with
neighborhoods that have received attention is the Traveling Salesman Problem;
e.g.\ see \cite{ah-aagcp-94,mm-aagtn-95,gl-faatn-99,dm-aatnp-01,delm-tsp-03,bgk+-tnvs-05,m-ptnfr-07}.
The bottleneck version of TSP is known to be NP-hard \cite[p.~212]{Garey_Johnson79}. 
A $2$-approximation has been known since 1984 \cite{parker_rardin84}.

Other work on geometric optimization with uncertainty regions has been
framed using the notions of imprecise data or neighborhoods. For
studies of shortest paths with uncertainty regions
see~\cite{pk-aspas-10,dmmw-rsprm-14,dmm-mspip-15}.  For a more general
treatment and discussion of problems such as convex hulls, see
L{\"o}ffler and van Kreveld~\cite{lv-lschi-10}, who also considered
the size of bounding boxs, diameters and related problems
in~\cite{lv-lbbsm-10}.  A discrete variant in $d$-dimensional space
was considered by Ding and Xu~\cite{dx-scccp-11}, who studied the
problem of picking one representative each from a family of finite
sets, such that the resulting set has a small enclosing
hypersphere. Fiala \emph{et al.}~\cite{fiala05} considered ``systems
of distant representatives'', which amounts to maximizing the minimum
distance between selected points. This is related to but different
from our work in this paper: we aim for minimizing the maximum length
in a spanning tree.

Another angle is to consider topological changes under uncertainty: when does the structure of an optimal solution change
when the input data is perturbed? Abellanas \emph{et al.}~\cite{ahr-stdt-99} studied this structure with respect to the largest 
perturbation of a set of planar points that keeps the Delaunay triangulation unchanged. Conversely, problems of determining
a necessary perturbation in order to achieve a desired change have also been studied; e.g., see Arkin \emph{et al.}\cite{adk+-ct-11}
for deciding whether a given set of neighborhoods has a convex stabber, which amounts to deciding whether a given set
can be moved into a convex position. For further discussions of related problems, see the excellent exposition by
L{\"o}ffler and van Kreveld~\cite{lv-lschi-10}.

\subsection{Our Main Results.}
After showing that several variants of BCU are NP-hard (some even to approximate), we give exact and approximation algorithms for certain variants.
%Best Case $\alpha$ settings
%and examine approximation algorithms for some of them.
%In our article, all distances are assumed to be Euclidean.
%As the underlying problem is inherently geometric in nature,
Given the geometric nature of our problems, we use the Euclidean measure of distance.
%focus our attention on Euclidean scenarios.
Our main results are as follows:
\begin{enumerate}
\item
We show that BCU is NP-hard even in the simple cases in which the uncertainty regions are point pairs and vertical line segments, respectively.
Our proof technique also works when the regions are all squares.
We further show that it is NP-hard to approximate BCU within a factor less than $\sqrt{5}/2$ when the uncertainty regions are pairs of points.
See Section~\ref{sec:hardness}.
\item
We present an exact algorithm for BCU when the instance consists of $n$ fixed points and $k$ line segments. The algorithm is polynomial in $n$ for constant $k$. The output of this algorithm is correct up to precision $\delta$, $\delta > 0$. See Section~\ref{sec:exactAlgorithm}.
\item
For uncertainty regions that are all unit disks, we give a simple constant additive approximation algorithm for BCU. A slight modification of this algorithm gives a constant multiplicative approximation in case the disks are \emph{non-overlapping}. See Section~\ref{sec:constant_factor_and_additive_approx}.
%For uncertainty regions that are all unit disks, we give constant additive approximation algorithms for $W\!\alpha$ and $B\alpha$.  The algorithm for $W\!\alpha$ is shown to be a constant (multiplicative) factor approximation while the $B\alpha$ algorithm is not.  However, a slight modification of the $B\alpha$ algorithm gives a constant multiplicative approximation in case the disks are \emph{non-overlapping}. See Section~\ref{sec:constant_factor_and_additive_approx}.
\item
We provide approximation results for the WCU. In particular, we establish methods with additive and multiplicative performance guarantees. See Section~\ref{sec:wcu}.
%We show constant additive approximation algorithms for $W\alpha$ and $B\alpha$, and a constant factor approximation algorithm for $B\alpha$, for the case where the uncertainty regions are non-overlapping (???) unit disks.
%\item
%We show that both $W\alpha$ and $B\alpha$ are in FPT when the instance consists of $n-k$ fixed points and $k$ pairs of points; the parameter is $k$.
\end{enumerate}


==> linkingGadgetSquares.tex <==
\begin{figure}[h]
\begin{center}
 \psset{unit=0.3cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
 \pspicture(0,0)(14,10)

 \psgrid[gridcolor=lightgray,subgriddiv=1,gridwidth=0.001pt,gridlabels=0pt](0,0)(0,0)(14,10)

 \psline(0,4)(1,4)(1,5)(0,5)(0,4)
 \psline(5,8)(4,8)(4,9)(5,9)(5,8)
 \psline(4,0)(5,0)(5,1)(4,1)(4,0)
 \psline(9,0)(10,0)(10,1)(9,1)(9,0)
 \psline(12,6)(13,6)(13,5)(12,5)(12,6)
 \psset{linecolor=\bluecolour}
 \pnode(4,10.5){a0}
 \dotnode(1,5){a1}
 \dotnode(4,9){a2}
 \dotnode(4,1){a3}
 \dotnode(9,1){a4}
 \dotnode(12,5){a5}
 \pnode(14,4.5){a6}
 \ncarc[arcangle=-30]{->}{a0}{a2}
 \ncline{->}{a2}{a1}
 \ncline{->}{a1}{a3}
 \ncarc[arcangle=30]{->}{a3}{a4}
 \ncline{->}{a4}{a5}
 \ncarc[arcangle=-30]{->}{a5}{a6}

 \psset{linecolor=\redcolour}
 \pnode(3.5,10){b0}
 \dotnode(1,4){b1}
 \dotnode(4,8){b2}
 \dotnode(5,1){b3}
 \dotnode(10,1){b4}
 \dotnode(13,5){b5}
 \pnode(14.5,5){b6}
 \ncarc[arcangle=-30]{<-}{b0}{b2}
 \ncline{<-}{b2}{b1}
 \ncline{<-}{b1}{b3}
 \ncarc[arcangle=30]{<-}{b3}{b4}
 \ncline{<-}{b4}{b5}
 \ncarc[arcangle=-30]{<-}{b5}{b6}
 \psset{linecolor=black}
 \endpspicture
\caption{An example corner gadget.}
\label{fig:linkgadget}
\end{center}
\end{figure}


==> prelims.tex <==
\RequirePackage{pstricks}
\RequirePackage{pst-node}
%
\newcommand{\qs}[1]{`#1'}
\newcommand{\fig}[4]{%
}


==> schema.tex <==
\begin{figure}[h]
\begin{center}
 \psset{unit=0.6cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
 \pspicture(-1,0.5)(11,7)
 \psline(1,0)(1,2)
 \psline(5,0)(5,2)
 \psline(9,0)(9,2)
 \psset{linecolor=gray,linewidth=1pt}
 \psline(2,4)(1,2)
 \psline(6,4)(5,2)
 \psline(10,4)(9,2)
 \psset{linecolor=gray,linestyle=dashed,linewidth=0.5pt}
 \psline(2,4)(0,4)
 \psline(6,4)(4,4)
 \psline(10,4)(8,4)
 \psarc(2,4){1}{180}{240}
 \psarc(6,4){1}{180}{240}
 \psarc(10,4){1}{180}{240}
 \psset{linecolor=black,linestyle=solid,linewidth=0.5pt}
 \psline(2,4)(4,4)
 \psline(6,4)(8,4)
 \psline(10,4)(11,4)(11,6)(-1,6)(-1,4)(0,4)
 \psdots(2,4)(0,4)(6,4)(4,4)(10,4)(8,4)(1,2)(5,2)(9,2)
 %
 \endpspicture
 \vspace*{10pt}
 \caption{Schema of the clause gadget. When a gray gate is open the
   entire clause gadget can be connected to the rest of the graph.}
\label{schema_clause_points}
\end{center}
\end{figure}


==> splittingGadgetSquares.tex <==
\begin{figure}[h]
\begin{center}
 \psset{unit=0.3cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
 \pspicture(4,-10)(19,11)
 \psline(4,0)(5,0)(5,1)(4,1)(4,0)
 \psline(9,0)(10,0)(10,1)(9,1)(9,0)
 \psline(14,0)(15,0)(15,1)(14,1)(14,0)
 \psline(18,-3)(19,-3)(19,-2)(18,-2)(18,-3)
 \psline(18,-8)(19,-8)(19,-7)(18,-7)(18,-8)
 \psline(18,4)(19,4)(19,5)(18,5)(18,4)
 \psline(18,9)(19,9)(19,10)(18,10)(18,9)
 \psset{linecolor=\bluecolour}
 \pnode(2.5,1){a1}
 \dotnode(4,1){a2}
 \dotnode(9,1){a3}
 \dotnode(14,1){a5}
 \dotnode(18,-2){a6}
 \dotnode(18,-7){a7}
 \pnode(17.5,-9){a75}
 \dotnode(18,4){a8}
 \dotnode(18,9){a9}
 \pnode(17.5,11){a95}
 \ncarc[arcangle=30]{->}{a1}{a2}
 \ncarc[arcangle=30]{->}{a2}{a3}
 \ncarc[arcangle=30]{->}{a3}{a5}
 \ncline{->}{a5}{a6}
 \ncarc[arcangle=-30]{->}{a6}{a7}
 \ncarc[arcangle=-30]{->}{a7}{a75}
 \ncline{->}{a5}{a8}
 \ncarc[arcangle=30]{->}{a8}{a9}
 \ncarc[arcangle=30]{->}{a9}{a95}

 \psset{linecolor=\redcolour}
 \pnode(3,1.5){b1}
 \dotnode(5,1){b2}
 \dotnode(10,1){b3}
 \dotnode(15,1){b5}
 \dotnode(18,-3){b6}
 \dotnode(18,-8){b7}
 \pnode(18,-10){b75}
 \dotnode(18,5){b8}
 \dotnode(18,10){b9}
 \pnode(18,12){b95}
 \ncarc[arcangle=30]{<-}{b1}{b2}
 \ncarc[arcangle=30]{<-}{b2}{b3}
 \ncarc[arcangle=30]{<-}{b3}{b5}
 \ncline{<-}{b5}{b6}
 \ncarc[arcangle=-30]{<-}{b6}{b7}
 \ncarc[arcangle=-30]{<-}{b7}{b75}
 \ncline{<-}{b5}{b8}
 \ncarc[arcangle=30]{<-}{b8}{b9}
 \ncarc[arcangle=30]{<-}{b9}{b95}
 \psset{linecolor=black}
 \endpspicture
\caption{Splitting the path from a variable to two (or more) clauses}
\label{fig:split}
\end{center}
\end{figure}


==> variableGadgetPoints.tex <==
\begin{figure}[h]
\begin{center}
% \psset{unit=0.45cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
 \psset{unit=0.3cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}
 \pspicture(0,-2)(38,14)

 \psline[linecolor=gray](6,-2)(6,14)
 \psline[linecolor=gray](14,-2)(14,14)
 \psline[linecolor=gray](18,-2)(18,14)
 \psline[linecolor=gray](26,-2)(26,14)
 \psline[linecolor=gray](34,-2)(34,14)

\rput(3,-2){$I$}
\rput(10,-2){$II$}
\rput(16,-2){$III$}
\rput(23,-2){$I$}
\rput(30,-2){$II$}
\rput(36,-2){$III$}

 \psset{linecolor=gray}
 \dotnode(0,6){a0}
 \dotnode(2,6){a1}
 \dotnode(4,6){a2}
 \dotnode(6,6){a3}
 \dotnode(6,4){a4}
 \dotnode(8,4){a5}
 \dotnode(10,4){a6}
 \dotnode(12,4){a7}
 \dotnode(14,4){a8}
 \dotnode(6,10){a9}
 \dotnode(8,10){a10}
 \dotnode(10,10){a11}
 \dotnode(12,10){a12}
 \dotnode(14,10){a13}
 \dotnode(14,0){a14}
 \dotnode(16,0){a15}
 \dotnode(18,0){a16}
 \dotnode(18,2){a17}
 \dotnode(18,4){a18}
 \dotnode(18,6){a19}
 \dotnode(18,8){a20}
 \dotnode(18,10){a21}
 \dotnode(18,12){a22}
 \dotnode(16,12){a23}
 \dotnode(14,12){a24}
 \dotnode(14,6){a25}
 \dotnode(16,6){a26}


 \dotnode(20,6){c0}
 \dotnode(22,6){c1}
 \dotnode(24,6){c2}
 \dotnode(26,6){c3}
 \dotnode(26,4){c4}
 \dotnode(28,4){c5}
 \dotnode(30,4){c6}
 \dotnode(32,4){c7}
 \dotnode(34,4){c8}
 \dotnode(26,10){c9}
 \dotnode(28,10){c10}
 \dotnode(30,10){c11}
 \dotnode(32,10){c12}
 \dotnode(34,10){c13}
 \dotnode(34,0){c14}
 \dotnode(36,0){c15}
 \dotnode(38,0){c16}
 \dotnode(38,2){c17}
 \dotnode(38,4){c18}
 \dotnode(38,6){c19}
 \dotnode(38,8){c20}
 \dotnode(38,10){c21}
 \dotnode(38,12){c22}
 \dotnode(36,12){c23}
 \dotnode(34,12){c24}
 \dotnode(34,6){c25}
 \dotnode(36,6){c26}

 \psset{linecolor=black,dotstyle=*}

 \dotnode(0,7){b0}
 \dotnode(2,7){b1}
 \dotnode(4,7){b2}
 \dotnode(6,7){b3}
 \dotnode(6,3){b4}
 \dotnode(8,3){b5}
 \dotnode(10,3){b6}
 \dotnode(12,3){b7}
 \dotnode(14,3){b8}
 \dotnode(6,9){b9}
 \dotnode(8,9){b10}
 \dotnode(10,9){b11}
 \dotnode(12,9){b12}
 \dotnode(14,9){b13}
 \dotnode(14,1){b14}
 \dotnode(16,1){b15}
 \dotnode(18,1){b16}
 \dotnode(18,3){b17}
 \dotnode(18,5){b18}
 \dotnode(18,7){b19}
 \dotnode(18,9){b20}
 \dotnode(18,11){b21}
 \dotnode(18,13){b22}
 \dotnode(16,13){b23}
 \dotnode(14,13){b24}
 \dotnode(14,7){b25}
 \dotnode(16,7){b26}

 \dotnode(20,7){d0}
 \dotnode(22,7){d1}
 \dotnode(24,7){d2}
 \dotnode(26,7){d3}
 \dotnode(26,3){d4}
 \dotnode(28,3){d5}
 \dotnode(30,3){d6}
 \dotnode(32,3){d7}
 \dotnode(34,3){d8}
 \dotnode(26,9){d9}
 \dotnode(28,9){d10}
 \dotnode(30,9){d11}
 \dotnode(32,9){d12}
 \dotnode(34,9){d13}
 \dotnode(34,1){d14}
 \dotnode(36,1){d15}
 \dotnode(38,1){d16}
 \dotnode(38,3){d17}
 \dotnode(38,5){d18}
 \dotnode(38,7){d19}
 \dotnode(38,9){d20}
 \dotnode(38,11){d21}
 \dotnode(38,13){d22}
 \dotnode(36,13){d23}
 \dotnode(34,13){d24}
 \dotnode(34,7){d25}
 \dotnode(36,7){d26}

 \psset{linecolor=black,nodesep=.1,linestyle=dashed,linewidth=1.5pt}
 \ncline{a0}{b0}
 \ncline{a1}{b1}
 \ncline{a2}{b2}
 \ncline{a3}{b3}
 \ncline{a4}{b4}
 \ncline{a5}{b5}
 \ncline{a6}{b6}
 \ncline{a7}{b7}
 \ncline{a8}{b8}
 \ncline{a9}{b9}
 \ncline{a10}{b10}
 \ncline{a11}{b11}
 \ncline{a12}{b12}
 \ncline{a13}{b13}
 \ncline{a14}{b14}
 \ncline{a15}{b15}
 \ncline{a16}{b16}
 \ncline{a17}{b17}
 \ncline{a18}{b18}
 \ncline{a19}{b19}
 \ncline{a20}{b20}
 \ncline{a21}{b21}
 \ncline{a22}{b22}
 \ncline{a23}{b23}
 \ncline{a24}{b24}
 \ncline{a25}{b25}
 \ncline{a26}{b26}

 \ncline{c0}{d0}
 \ncline{c1}{d1}
 \ncline{c2}{d2}
 \ncline{c3}{d3}
 \ncline{c4}{d4}
 \ncline{c5}{d5}
 \ncline{c6}{d6}
 \ncline{c7}{d7}
 \ncline{c8}{d8}
 \ncline{c9}{d9}
 \ncline{c10}{d10}
 \ncline{c11}{d11}
 \ncline{c12}{d12}
 \ncline{c13}{d13}
 \ncline{c14}{d14}
 \ncline{c15}{d15}
 \ncline{c16}{d16}
 \ncline{c17}{d17}
 \ncline{c18}{d18}
 \ncline{c19}{d19}
 \ncline{c20}{d20}
 \ncline{c21}{d21}
 \ncline{c22}{d22}
 \ncline{c23}{d23}
 \ncline{c24}{d24}
 \ncline{c25}{d25}
 \ncline{c26}{d26}

 \psset{linecolor=gray,nodesep=.1pt,linestyle=solid,linewidth=0.5pt,arrows=->}
\psset{arcangle=-8}
 \ncarc{a0}{a1}
 \ncarc{a1}{a2}
 \ncarc{a2}{a3}
 \ncarc{a3}{a4}
\psset{arcangle=8}
 \ncarc{a4}{a5}
 \ncarc{a5}{a6}
 \ncarc{a6}{a7}
 \ncarc{a7}{a8}
 \ncarc{a8}{a25}
\psset{arcangle=-8}
 \ncarc{a25}{a26}
 \ncarc{a26}{a19}
\psset{arcangle=-40}
 \ncarc{a19}{a20}
 \ncarc{a20}{a21}
 \ncarc{a21}{a22}
\psset{arcangle=8}
 \ncarc{a22}{a23}
 \ncarc{a23}{a24}
 \ncarc{a24}{a13}
\psset{arcangle=-8}
 \ncarc{a13}{a12}
 \ncarc{a12}{a11}
 \ncarc{a11}{a10}
 \ncarc{a10}{a9}
 \ncarc{a19}{c0}
 \ncarc{c0}{c1}
 \ncarc{c1}{c2}
 \ncarc{c2}{c3}
 \ncarc{c3}{c4}
\psset{arcangle=8}
 \ncarc{c4}{c5}
 \ncarc{c5}{c6}
 \ncarc{c6}{c7}
 \ncarc{c7}{c8}
 \ncarc{c8}{c25}
\psset{arcangle=-8}
 \ncarc{c25}{c26}
 \ncarc{c26}{c19}
\psset{arcangle=-40}
 \ncarc{c19}{c20}
 \ncarc{c20}{c21}
 \ncarc{c21}{c22}
\psset{arcangle=8}
 \ncarc{c22}{c23}
 \ncarc{c23}{c24}
 \ncarc{c24}{c13}
\psset{arcangle=-8}
 \ncarc{c13}{c12}
 \ncarc{c12}{c11}
 \ncarc{c11}{c10}
 \ncarc{c10}{c9}
 \endpspicture
\caption{An example variable gadget.}
\label{vble_gadget_points}
\end{center}
\end{figure}

==> variableGadgetSquares.tex <==
\begin{figure}[h]
\begin{center}
 \psset{unit=0.3cm,arrows=-,shortput=nab,linewidth=0.5pt,arrowsize=2pt 5,labelsep=5.5pt}

 \pspicture(-1,-1)(38,26)

 \psgrid[gridcolor=lightgray,subgriddiv=1,gridwidth=0.001pt,gridlabels=0pt](0,0)(-1,-1)(38,26)

 \psline(13,0)(14,0)(14,1)(13,1)(13,0)
 \psline(23,0)(24,0)(24,1)(23,1)(23,0)
 \psline(4,3)(5,3)(5,4)(4,4)(4,3)
 \psline(9,3)(10,3)(10,4)(9,4)(9,3)
 \psline(27,3)(28,3)(28,4)(27,4)(27,3)
 \psline(32,3)(33,3)(33,4)(32,4)(32,3)
 \psline(0,7)(1,7)(1,8)(0,8)(0,7)
 \psline(13,7)(14,7)(14,8)(13,8)(13,7)
 \psline(18,7)(19,7)(19,8)(18,8)(18,7)
 \psline(23,7)(24,7)(24,8)(23,8)(23,7)
 \psline(36,7)(37,7)(37,8)(36,8)(36,7)
 \psline(0,12)(1,12)(1,13)(0,13)(0,12)
 \psline(36,12)(37,12)(37,13)(36,13)(36,12)
 \psline[linewidth=1.5pt](4,17)(5,17)(5,18)(4,18)(4,17)
 \psline(13,17)(14,17)(14,18)(13,18)(13,17)
 \psline(18,17)(19,17)(19,18)(18,18)(18,17)
 \psline(23,17)(24,17)(24,18)(23,18)(23,17)
 \psline(36,17)(37,17)(37,18)(36,18)(36,17)
 \psline(9,21)(10,21)(10,22)(9,22)(9,21)
 \psline(27,21)(28,21)(28,22)(27,22)(27,21)
 \psline(32,21)(33,21)(33,22)(32,22)(32,21)
 \psline(13,24)(14,24)(14,25)(13,25)(13,24)
 \psline(23,24)(24,24)(24,25)(23,25)(23,24)

 \psdots[linecolor=\bluecolour](13,1)(24,0)(4,4)(9,4)(27,4)(32,4)(1,8)(13,7)(18,7)(23,7)(36,7)(1,13)(36,12)(4,17)(14,18)(19,18)(24,18)(36,17)(10,21)(28,21)(33,21)(13,25)(24,24)
 \psdots[linecolor=\redcolour](13,0)(24,1)(5,4)(10,4)(28,4)(33,4)(1,7)(14,7)(19,7)(24,7)(36,8)(1,12)(36,13)(5,18)(13,18)(18,18)(23,18)(36,18)(9,21)(27,21)(32,21)(13,24)(24,25)

 \pnode(13,1){b1}
 \pnode(13.5,-1){b1x}
 \pnode(24,0){b2}
 \pnode(23.5,-2){b2x}
 \pnode(4,4){b3}
 \pnode(9,4){b4}
 \pnode(27,4){b5}
 \pnode(32,4){b6}
 \pnode(1,8){b7}
 \pnode(13,7){b8}
 \pnode(18,7){b9}
 \pnode(23,7){b10}
 \pnode(36,7){b11}
 \pnode(1,13){b12}
 \pnode(36,12){b15}
 \pnode(4,17){b16}
 \pnode(14,18){b17}
 \pnode(19,18){b18}
 \pnode(24,18){b19}
 \pnode(36,17){b20}
 \pnode(10,21){b21}
 \pnode(28,21){b22}
 \pnode(33,21){b23}
 \pnode(13,25){b24}
 \pnode(13.5,27){b24x}
 \pnode(24,24){b25}
 \pnode(23.5,26){b25x}

 \pnode(13,0){r1}
 \pnode(12.5,-2){r1x}
 \pnode(24,1){r2}
 \pnode(24.5,-1){r2x}
 \pnode(5,4){r3}
 \pnode(10,4){r4}
 \pnode(28,4){r5}
 \pnode(33,4){r6}
 \pnode(1,7){r7}
 \pnode(14,7){r8}
 \pnode(19,7){r9}
 \pnode(24,7){r10}
 \pnode(36,8){r11}
 \pnode(1,12){r14}
 \pnode(36,13){r15}
 \pnode(5,18){r16}
 \pnode(13,18){r17}
 \pnode(18,18){r18}
 \pnode(23,18){r19}
 \pnode(36,18){r20}
 \pnode(9,21){r21}
 \pnode(27,21){r22}
 \pnode(32,21){r23}
 \pnode(13,24){r24}
 \pnode(12.5,26){r24x}
 \pnode(24,25){r25}
 \pnode(24.5,27){r25x}

 \psset{linecolor=\bluecolour}
 \ncline{->}{b16}{b12}
 \ncarc[arcangle=30]{->}{b14}{b12}
 \ncarc[arcangle=30]{->}{b12}{b7}
 \ncline{->}{b7}{b3}
 \ncarc[arcangle=30]{->}{b3}{b4}
 \ncline{->}{b4}{b1}
 \ncline{->}{b4}{b8}
 \ncarc[arcangle=30]{->}{b8}{b9}
 \ncarc[arcangle=30]{->}{b9}{b10}
 \ncline{->}{b10}{b5}
 \ncarc[arcangle=30]{->}{b5}{b6}
 \ncline{->}{b6}{b11}
 \ncarc[arcangle=30]{->}{b11}{b15}
 \ncarc[arcangle=30]{->}{b15}{b20}
 \ncline{->}{b20}{b23}
 \ncarc[arcangle=30]{->}{b23}{b22}
 \ncline{->}{b22}{b19}
 \ncline{->}{b22}{b25}
 \ncarc[arcangle=30]{->}{b19}{b18}
 \ncarc[arcangle=30]{->}{b18}{b17}
 \ncline{->}{b17}{b21}
 \ncline{->}{b24}{b21}
 \ncline{->}{b2}{b5}
 \ncarc[arcangle=30]{->}{b24x}{b24}
 \ncarc[arcangle=30]{->}{b25}{b25x}
 \ncarc[arcangle=30]{->}{b1}{b1x}
 \ncarc[arcangle=30]{->}{b2x}{b2}

 \psset{linecolor=\redcolour}
 \ncline{->}{r16}{r21}
 \ncline{->}{r21}{r24}
 \ncline{->}{r21}{r17}
 \ncarc[arcangle=30]{->}{r17}{r18}
 \ncarc[arcangle=30]{->}{r18}{r19}
 \ncline{->}{r19}{r22}
 \ncline{->}{r25}{r22}
 \ncarc[arcangle=30]{->}{r22}{r23}
 \ncline{->}{r23}{r20}
 \ncarc[arcangle=30]{->}{r20}{r15}
 \ncarc[arcangle=30]{->}{r15}{r11}
 \ncline{->}{r11}{r6}
 \ncarc[arcangle=30]{->}{r6}{r5}
 \ncline{->}{r5}{r2}
 \ncline{->}{r5}{r10}
 \ncarc[arcangle=30]{->}{r10}{r9}
 \ncarc[arcangle=30]{->}{r9}{r8}
 \ncline{->}{r8}{r4}
 \ncline{->}{r1}{r4}
 \ncarc[arcangle=30]{->}{r4}{r3}
 \ncline{->}{r3}{r7}
 \ncarc[arcangle=30]{->}{r7}{r14}
 \ncarc[arcangle=30]{->}{r24}{r24x}
 \ncarc[arcangle=30]{->}{r25x}{r25}
 \ncarc[arcangle=30]{->}{r1x}{r1}
 \ncarc[arcangle=30]{->}{r2}{r2x}

 \endpspicture
\end{center}
\caption{An example variable gadget.}
\label{fig:variablegadget}
\end{figure}

